Offline Reinforcement Learning: Role of State Aggregation and Trajectory Data

We revisit the problem of offline reinforcement learning with value function realizability but without Bellman completeness. Previous work by Xie and Jiang (2021) and Foster et al. (2022) left open the question whether a bounded concentrability coefficient along with trajectory-based offline data admits a polynomial sample complexity. In this work, we provide a negative answer to this question for the task of offline policy evaluation. In addition to addressing this question, we provide a rather complete picture for offline policy evaluation with only value function realizability. Our primary findings are threefold: 1) The sample complexity of offline policy evaluation is governed by the concentrability coefficient in an aggregated Markov Transition Model jointly determined by the function class and the offline data distribution, rather than that in the original MDP. This unifies and generalizes the ideas of Xie and Jiang (2021) and Foster et al. (2022), 2) The concentrability coefficient in the aggregated Markov Transition Model may grow exponentially with the horizon length, even when the concentrability coefficient in the original MDP is small and the offline data is admissible (i.e., the data distribution equals the occupancy measure of some policy), 3) Under value function realizability, there is a generic reduction that can convert any hard instance with admissible data to a hard instance with trajectory data, implying that trajectory data offers no extra benefits over admissible data. These three pieces jointly resolve the open problem, though each of them could be of independent interest.

==> files/admissible_lb_example.tex <==
\section{Proof of \pref{thm:admissible}}  \label{app: admissible lb}
\par In this subsection, we will prove \pref{thm:admissible}. Actually we will prove the following stronger results about $(Q, W)$-realizability:
\begin{theorem}\label{thm:admissible-stronger}
    For any $\epsilon\le \nicefrac{1}{6}$ There exists a class $\mathcal{M}$ of $H$-layer MDPs with shared state spaces and action spaces, and two policies $\pieval$ and $\piexp$, such that for any $N = o(2^{H-6}\nicefrac{H^3}{\epsilon})$,
    \begin{itemize}
        \item the concentrability coefficient of policy $\pieval$ with respect to $d_h^\piexp$ is upper bounded by $48H^2$;
        \item the (Q, W)-function class 
        $$\{(Q^\pieval(\cdot, \cdot~; M), W(\cdot; d^\piexp(\cdot; M); M)): M\in\mathcal{M}\}$$
        has only two elements;
        \item For size $N$ admissible data $\mathcal{D}(M)$ with respect to policy $\pieval$ from MDP $M\in \mathcal{M}$: $\mathcal{D}(M) = \cup_{h=1}^H \mathcal{D}_h(M)$ where
        $$\mathcal{D}_h(M) = \{(\sx_h^i, \sa_h^i, r_h^i, \sx_{h+1}^i)_{i=1}^N: (\sx_h^i, \sa_h^i)\sim d_h^\piexp(\cdot), r_h^i\sim R(\cdot \mid \sx, \sa; M), \sx_{h+1}^i\sim T(\cdot\mid \sx, \sa; M)\},$$
        any algorithm which takes $\mathcal{D}(M)$ as input and output the evaluation of value function $V^\pieval(\rho; M)$ cannot achieve $\nicefrac{\epsilon}{H}$-accurate for all $M\in\mathcal{M}$ with probability at least $\nicefrac{1}{2}$.
    \end{itemize}
\end{theorem}
We construct the Markov Transition Model $M = (\cZ, \cA, T, H, \rho)$ as
\begin{enumerate}[label=\(\bullet\)] 
\item \textbf{State space} $\calZ = \cup_{h=1}^H \calZ_h$, where $\calZ_h = \{\sz_h\inds{1}, \sz_h\inds{2}, \sz_h\inds{3}\}$.

\item \textbf{Action space} $\calA = \{a_1, a_2\}$.

\item \textbf{Transition model} $T$ is defined as 
\begin{align*}
    T(\sz'\mid \sz, \sa) = \begin{cases}
        1/2\quad & \sz = \sz_h\inds{1}, \sa = \sa_1\quad \text{or}\quad \sz = \sz_h\inds{2}, \sa = \sa_2, \sz' = \sz_{h+1}\inds{1},\\
        1\quad & \sz = \sz_h\inds{3}, \sz'= \sz_{h+1}\inds{3}\quad \text{or}\quad \sz = \sz_h\inds{2}, \sa = \sa_1, \sz' = \sz_{h+1}\inds{3},\\
        \frac{H-2}{2H-2} & \sz = \sz_h\inds{1}, \sa = \sa_2, \sz' = \sz_{h+1}\inds{1}\quad \text{or}\quad \sz = \sz_h\inds{2}, \sa = \sa_2, \sz' = \sz_{h+1}\inds{3},\\
        \frac{H}{2H-2} & \sz = \sz_h\inds{1}, \sa = \sa_2, \sz' = \sz_{h+1}\inds{3},\\
        \frac{1}{2H-2} &\sz = \sz_h\inds{2}, \sa = \sa_2, \sz' = \sz_{h+1}\inds{2},\\
        0 &\text{otherwise}.
    \end{cases}
\end{align*}

%\ascomment{Make the above a case block similar to before}

\item \textbf{Initial distribution} $\rho$ is defined as 
$$\rho(\cdot) = \frac{H-1}{2H}\delta_{\sz_1\inds{1}}(\cdot) + \frac{1}{2H}\delta_{\sz_1\inds{2}}(\cdot) + \frac{1}{2}\delta_{\sz_1\inds{3}}(\cdot)$$
\end{enumerate}

Additionally, we further define
\begin{itemize}
    \item \textbf{Policy to be evaluated} $\pieval(\cdot) = \delta(a_1)$.
    \item \textbf{Offline Data Collection Policy} $\piexp = \frac{1}{H}\delta\prn{\sa_1} + \frac{H-1}{H}\delta\prn{\sa_2}$.    
    \item \textbf{Aggregation scheme} $\Phi = \cup_{h=1}^H \{\phi_h\inds{1}, \phi_h\inds{2}\}$ with $\phi_h\inds{1} = \{\sz_h\inds{1}, \sz_h\inds{2}\}, \phi_h\inds{2} = \{\sz_h\inds{3}\}$.
\end{itemize}

For this MDP and data collection distribution, we have the following propositions:

\begin{lemma}\label{lem:sec-admissible-mu} For MDP \(M\), and policy $\piexp$ defined above. If we let $\mu_h(\cdot) \ldef{}  d_h^\piexp(\cdot; M)$, then we have 
$$\mu_h(\sz_h\inds{1}, \sa_1) = \frac{H-1}{2^h H^2}, \quad \mu_h(\sz_h\inds{2}, \sa_1) = \frac{1}{2^h H^2} \quad\text{and}\quad \mu_h(\sz_h\inds{3}, \sa_1) = \frac{2^h - 1}{2^h H},\quad \forall 1\le h\le H.$$
\end{lemma}
\begin{proofof}[\pref{lem:sec-admissible-mu}]
    By calculation, we find out that under policy $\piexp$, the transition satisfies
    \begin{align*}
        T(\cdot\mid \sz_h\inds{1}, \piexp(\sz_h\inds{1})) = T(\cdot\mid \sz_h\inds{2}, \piexp(\sz_h\inds{2}))& = \frac{H-1}{2H}\delta_{\sz_{h+1}\inds{1}}(\cdot) + \frac{1}{2H}\delta_{\sz_{h+1}\inds{2}}(\cdot) + \frac{1}{2}\delta_{\sz_{h+1}\inds{3}}(\cdot),\\
        T(\cdot\mid \sz_h\inds{3}, \piexp(\sz_h\inds{3})) & = \delta_{\sz_{h+1}\inds{3}}(\cdot).
    \end{align*}
    Hence according to the initial distribution $\rho(\cdot) = \frac{H-1}{2H}\delta_{\sz_1\inds{1}}(\cdot) + \frac{1}{2H}\delta_{\sz_1\inds{2}}(\cdot) + \frac{1}{2}\delta_{\sz_1\inds{3}}(\cdot)$, we have
    \begin{equation}\label{eq:sec-lower-bound-dpiexp}
        d_h^\piexp(\sz_h\inds{1}; M) = \frac{H-1}{2^hH}, \quad d_h^\piexp(\sz_h\inds{2}; M) = \frac{1}{2^h H} \quad\text{and}\quad d_h^\piexp(\sz_h\inds{3}; M) = \frac{2^h - 1}{2^h} \quad \forall 1\le h\le H.
    \end{equation}
    Next, since the exploration policy $\piexp$  is chosen to be $\piexp(\cdot) = \frac{1}{H}\delta_{\sa_1}(\cdot) + \frac{H-1}{H}\delta_{\sa_2}(\cdot)$, we have
    \begin{align*}
        \mu_h(\sz_h\inds{1}, \sa_1) = \frac{H-1}{2^h H^2}, \quad \mu_h(\sz_h\inds{2}, \sa_1) = \frac{1}{2^h H^2} \quad\text{and}\quad \mu_h(\sz_h\inds{3}, \sa_1) = \frac{2^h - 1}{2^h H}. 
    \end{align*} 
\end{proofof}

\begin{lemma}\label{lem:admissible-c} For the MDP \(M\), and offline distribution \(\mu\)  induced by policy \(\piexp\) defined above, the concentrability coefficient of policy $\pieval$ with respect to distribution $\mu$ is upper bounded as 
\begin{align*}
    C(M; \mu) = \max_{h}\max_{\sz\in\calZ_h}\frac{d_h^\pieval(\sz; M)}{\mu_h(\sz, \pieval(\sz))}\le H^2
\end{align*}
However, for $\epsilon\le \nicefrac{1}{6}$, the aggregated concentrability coefficient is lower bounded as
\begin{align*}
    \ophatC{M}{\Phi}{\mu}{\epsilon}\ge 2^{H-3} H.
\end{align*}
\end{lemma}
\begin{proofof}[\pref{lem:admissible-c}]
    For the upper bound of $C(M; \mu)$, by calculation, we have that under policy $\piexp$, the transition satisfies
    \begin{align*}
        T(\cdot\mid \sz_h\inds{1}, \pieval(\sz_h\inds{1}))& = \frac{1}{2}\delta_{\sz_{h+1}\inds{1}}(\cdot) + \frac{1}{2}\delta_{\sz_{h+1}\inds{2}}(\cdot),\\
        T(\cdot\mid \sz_h\inds{2}, \pieval(\sz_h\inds{2})) & = \delta_{\sz_{h+1}\inds{3}}(\cdot),\\
        T(\cdot\mid \sz_h\inds{3}, \pieval(\sz_h\inds{3})) & = \delta_{\sz_{h+1}\inds{3}}(\cdot).
    \end{align*} 
    Hence the initial distribution $\rho(\cdot) = \frac{H-1}{2H}\delta_{\sz_1\inds{1}}(\cdot) + \frac{1}{2H}\delta_{\sz_1\inds{2}}(\cdot) + \frac{1}{2}\delta_{\sz_1\inds{3}}(\cdot)$ gives that for any $2\le h\le H$,
    $$d_h^\pieval(\sz_h\inds{1}; M) = d_h^\pieval(\sz_h\inds{2}; M) = \frac{H-1}{H\cdot 2^h},\quad d_h^\pieval(\sz_h\inds{2}; M) = 1 - \frac{H-1}{H\cdot 2^{h-1}}.$$
    Hence according to \pref{lem:sec-admissible-mu}, we have for $2\le h\le H$,
    $$\max_{\sz\in\calZ_h}\frac{d_h^\pieval(\sz; M)}{\mu_h(\sz, \pieval(\sz))}\le H^2,$$
    and for $h = 1$, we have $d_h^\pieval(\sz; M) = \mu_h(\sz, \pieval(\sz)) = \rho(\sz)$ for any $\sz\in\calZ_1$, hence 
    $$\max_{\sz\in\calZ_h}\frac{d_h^\pieval(\sz; M)}{\mu_h(\sz, \pieval(\sz))} = 1.$$
    Above all, we get
    $$\tabC(M, \mu) = \max_{h}\max_{\sz\in\calZ_h}\frac{d_h^\pieval(\sz; M)}{\mu_h(\sz, \pieval(\sz))}\le H^2.$$


    As for the lower bound of $\ophatC{M}{\Phi}{\mu}{\epsilon}$, according to \pref{eq:agg-transition-model} and also our choice of $\mu$,
    \begin{align*}
        &\agg{T}(\phi_{h+1}\inds{1}\mid \phi_h\inds{1}, \sa_1) = \frac{\sum_{\sz_h\in\phi_h\inds{1}, \sz_{h+1}'\in\phi_{h+1}\inds{1}}\mu(\sz_h, \sa_1)T(\sz_{h+1}'\mid \sz_h, \sa_1)}{\sum_{\sz\in\phi_h\inds{1}}\mu(\sz, \sa_1)} \\ 
        &\qquad\ge \frac{\sum_{\sz_{h+1}'\in\phi_{h+1}\inds{1}}\mu(\sz_h\inds{1}, \sa_1)T(\sz_{h+1}'\mid \sz_h\inds{1}, \sa_1)}{\sum_{\sz\in\phi_h\inds{1}}\mu(\sz, \sa_1)}= \frac{\mu(\sz_h\inds{1}, \sa_1)}{\sum_{\sz\in\phi_h\inds{1}}\mu(\sz, \sa_1)} = \frac{H-1}{H-1 + 1} = \frac{H-1}{H}.
    \end{align*}
    Since $\pieval(\sz) = \delta(\sa_1)$ for all $\sz$, this implies that $\agg{d}_H^\pieval(\phi_H\inds{1}; M)$ satisfies
    \begin{align*}
        \agg{d}_H^\pieval(\phi_H\inds{1}; M)\ge \agg{d}_1^\pieval(\phi_1\inds{1}; M)\prod_{h=1}^{H-1}\agg{T}(\phi_{h+1}\inds{1}\mid \phi_h\inds{1}, \sa_1)\ge \frac{1}{2}\left(\frac{H-1}{H}\right)^{H-1}\ge \frac{1}{2e}\ge \frac{1}{6}.
    \end{align*}
    Hence when $\epsilon\le \nicefrac{1}{6}$, we have
    \begin{align*}
        \ophatC{M}{\Phi}{\mu}{\epsilon}\ge \frac{\agg{d}_H^\pieval(\phi_H\inds{1}; M)}{\sum_{\sz\in \phi_H\inds{1}}\mu(\sz, \pieval(\sz))} = \frac{\agg{d}_H^\pieval(\phi_H\inds{1}; M)}{\mu(\sz_H\inds{1}, \pieval(\sz_H\inds{1})) + \mu(\sz_H\inds{2}, \pieval(\sz_H\inds{2}))}\ge \frac{\nicefrac{1}{6}}{\nicefrac{1}{(H\cdot 2^H)}}\ge 2^{H-3}H.
    \end{align*}
\end{proofof}




\subsection{Proof of \pref{thm:admissible}}
\iffalse
\ascomment{\begin{enumerate}
\item First define the family. 
\item Then, mention that you will construct the class of MDPs using this family. 
\item Define the class of MDPs. 
\item All of the above should be quick since we operate at class level (no need to define state space, etc). 
\item Mention that all MDPS  have bounded C. 
\item Uncomment the picture. 
\end{enumerate}
}
\fi



\begin{proofof}[\pref{thm:admissible}]
    We consider the class of offline RL problems constructed in \pref{app:family_construction}: $\mathfrak{G} = \bigcup_{\psi \in \Psi} \crl{\mathfrak{g}\ind{1}_\psi,\mathfrak{g}\ind{2}_\psi}$. According to the construction, the sampling distributions over rich observations in $\mathfrak{g}\ind{1}_\psi$ or $\mathfrak{g}\ind{2}_\psi$ are $\rich{\mu}_\psi(\sx, \sa) = \nicefrac{\mu(\psi(\sz), \sa)}{|\calX_\psi(\sz)|}$. And \pref{thm:stronger} indicates that for $\epsilon\le \nicefrac{1}{6}$, for any algorithm using less than
    $$\frac{H\ophatC{M}{\phi}{\mu}{\epsilon}}{8\epsilon}\ge 2^{H-6}\frac{H^3}{\epsilon}$$
    samples, there must exist some $\psi\in\Phi$ such that if the samples are according to $\rich{\mu}_\psi$, the algorithm will have error greater than $\nicefrac{\epsilon}{8H}$ in $\mathfrak{g}\ind{1}_\psi$ or $\mathfrak{g}\ind{2}_\psi$ with probability at least $\nicefrac{1}{2}$.

    \par Our next observation is that according to \pref{lem:sec-lower-bound-latent-MDP} \ref{lem:sec-lower-bound-latent-MDP-d},
    we have $d^\piexp(\sz; M\ind{1})\le d^\piexp(\sz; M)$ for any $\sz\in\calZ$. Hence we obtain that for any $\sx\in\calX\backslash \{\su, \sv, \sw\}_{h=1}^H$,
    $$d^{\ripiexp}(\sx; \rich{M}_\psi\ind{1}) = \frac{d^\piexp(\psi(\sx); M)}{|\calX_\psi(\sz)|}\le \frac{d^\piexp(\psi(\sx); M)}{|\calX_\psi(\sz)|}.$$
    This also implies
    $$d^{\ripiexp}(\sx, \sa; \rich{M}_\psi\ind{1}) = d^{\ripiexp}(\sx; \rich{M}_\psi\ind{1})\piexp(\sa\mid\sx)\le \frac{d^\piexp(\psi(\sx); M)\piexp(\sa\mid\sx)}{|\calX_\psi(\sz)|} = \frac{d^\piexp(\psi(\sx), \sa; M)}{|\calX_\psi(\sz)|} = \rich{\mu}_\psi(\sx, \sa).$$
    Similarly, we can also obtain that
    $$d^{\ripiexp}(\sx, \sa; \rich{M}_\psi\ind{2})\le \rich{\mu}_\psi(\sx, \sa).$$
    Hence for any algorithm using less than $\nicefrac{2^{H-6}H^3}{\epsilon}$ number of samples, there must exists some $\rich{M}\in \{\rich{M}_\psi\ind{1}: \psi\in\Psi\}\cup\{\rich{M}_\psi\ind{2}: \psi\in\Psi\}$ such that if the samples are according to $d^{\ripiexp}(\cdot \mid \rich{M})$, the estimation error is at least $\nicefrac{\epsilon}{(8H)}$.

    \par Finally, \pref{lem:admissible-c} indicates that the concentrability coefficient of $M$ is bounded by $H^2$. Hence according to \pref{lem:sec-lower-bound-latent-MDP} \ref{lem:sec-lower-bound-latent-MDP-d} and \pref{corr:sec-lower-bound-d-pi} we have for any such $\rich{M}$, the concentrability coefficient is upper bounded by $48H^2$. And similar to the proof of \pref{thm:stronger}, we can also show that the class of $(Q, W)$-functions contains only two items.
\end{proofof}

% FIGURE HIDDEN 
% \begin{figure}
%    \caption{Hard Case for Admissible Data}
%    \label{fig:MDP}
%    \centering
%    \includegraphics[width = \textwidth]{figures/admissible.jpg}
% \end{figure}
%
\clearpage 



==> files/app_trajectory_offline.tex <==
\subsection{Lower Bound for Trajectory Data} \label{sec: trajectory lower bound} 
  
In \pref{sec: admissible data}, we showed that bounded concentrability coefficient and realizability are not sufficient for statistically tractable offline RL, even if the offline dataset of tuples \((\sx, \sa, \sr, \sx') \sim d^\piexp\) is admissible. However, in many real applications, the offline dataset is collected by sampling trajectories of the form \((\sx_1, \sa_1, \sr_1, \sx_2,  \dots, \sx_{H}, \sa_{H}, \sr_{H})\) and it remains to address whether access to the entire \(H\)-length trajectory instead of just the tuples \((\sx, \sa, \sr, \sx')\) could allow a learner to circumvent the challenges introduced in previous subsections. In fact, understanding the role of trajectory data is left open as an open problem by \citet{foster2022offline}.  In this section, we answer this in the negative and show that in the worst case, access to trajectory data does not allow for statistically efficient offline RL under just bounded concentrability coefficient and realizability. Our main result in this section is as follows, whose proof is deferred to \pref{app: proof of reduction}.

\begin{theorem}
\ascomment{This also needs to be changed to a class of offline policy evaluation problems!} 
    There exists a class of MDPs with bounded concentrability coefficient $64H$, and any algorithm using $o(\exp(H/4))$ trajectories together with realizable $Q$-function class induces estimation error $\nicefrac{\epsilon}{16H}$ in at least one MDP.
\end{theorem}

The proof of  \pref{thm:trajectory_lower_bound} follows from combining the result of \pref{thm:admissible} with a general purpose reduction from offline RL with admissible data to offline RL with trajectory data, which may be of independent interest. The reduction is based on a \Replicator-gadget, described below, that converts an \MDP $M = \MDP(\calX, \calA, T, r, H, \rho)$ into an \MDP  $\wt M = \MDP(\wt\calX, \calA, \wt T, \wt r, \wt H, \wt\rho)$ where \(\wt H = (H-1)K + 1\) by replicating each layer in \(M\) for \(K\) many  layers. In addition to the \Replicator-gadget, we also provide: 
\begin{enumerate}[label=\(\bullet\)] 
\item Protocols to lift offline distribution \(\pioff\), evaluation policy \(\pieval,\) and function class \(\cF\) (that realizes \(Q^{\pieval}\)) for the  \MDP \(M\) into corresponding offline distribution \(\wtpioff\), evaluation policy \(\wtpieval,\) and function class \(\wt \cF\) (that realizes \(Q^{\wtpieval}\)) for the lifted \MDP \(\wt M\). 
 
\item An \converter~protocol (given in \pref{alg:convert}):  that takes as input an admissible dataset \(\cD_h\) for each \(h \in [H]\), each consisting of $K$ tuples of the form \((\sx, \sa, \sr, \sx') \sim d_h^{\pioff}\), and outputs  a trajectory \(\tau\) of length~\(\wt H\). 
\end{enumerate} 

\paragraph{\Replicator-gadget, and related lifting operators.} The \Replicator-gadget replaces each layer of the \MDP \(M\) by \(K\) new layers by replicating the state space space \(K\) times. To simplify the notation, we assume that we replace a state \(\sx \in \cX_h\) in \(M\) by states \((\sx, 1), \dots, (\sx, K)\) in \(\wt M\) from layers \((h-1)K + 1\) to layers  \(hK\)  respectively. The transition dynamics within the buffers are given by: 
\begin{itemize}
\item \textit{When \(k \leq K-1\):} From a state \((\sx, k)\) on taking an action \(a\), transition to a state \((\sx', k+1)\) where  
\begin{align*}
\sx' \sim \begin{cases}
    \delta(\sx) & \text{if} \quad a = \pieval(\sx) \\ 
    d_h^{\pieval} & \text{if} \quad a \neq \pieval(\sx)
\end{cases},   
\end{align*} 
where \(d_h^{\pieval}\) denotes the occupancy measure of \(\pieval\) at layer \(h\) in \(M\). 
  
\item \textit{When \(k = K\):} From any state \((\sx, K)\), on taking an action \(a\), transition to \((\sx', 1)\) (corresponding to the next buffer) where \(\sx' \in \cX_{h+1}\) and is sampled as 
\begin{align*}
\sx' \sim T(\cdot \mid \sx, a). 
\end{align*}
\end{itemize} 
Finally, the reward function is given by $\wt r((\sx, k), \sa) = r(\sx, \sa) \indic\crl{k = K}$, and the initial distribution $\wt{\rho}((\sx, 1)) = \rho(\sx)$, $\wt{\rho}((\sx, k)) = 0$ for any $2\le k\le K$. 

Furthermore, the policy $\wtpieval$ to be evaluated is defined as: $\wtpieval((\sx, k)) = \pieval(\sx)$, and the policy $\wtpiexp$ used as a proxy from \(\pieval\) in \(\wt M\) is defined as:
$$\wtpiexp((\sx, k)) = \begin{cases}
\frac{1}{2}\pieval(\sx) + \frac{1}{2}\piother(\sx) &\quad \text{if } \quad 1\leq k\leq K-1, \\
    \piexp(\sx) &\quad \text{if } \quad k = K,  
\end{cases}$$ 
where $\piother(\cdot)$ is a policy such that $\piother(\sx)\neq \pieval(\sx)$. 

\paragraph{Intuition for \converter{}.} Due to above lifting, when the chosen action on \((\sx, k)\) is identical to the one chosen by \(\pieval\) (on \(\sx\) in \(M\)) for \(k \leq K-1\), the next state will be \((\sx, k+1)\), and thus the trajectory can be easily constructed. On the other hand, deviating from \(\wtpieval\) will immediately results in transitioning to a freshly sampled state from \(d_{h+1}^{\pioff}\); and again the trajectory can be easily simulated by mapping this transition to a random state \(\sx\) in \(\cD_{h+1}\) which contains tuples $(\sx, \sa, \sr, \sx')$, where \(\sx \sim d_{h+1}^{\pioff}\). In fact, we have the following lemma. 
\begin{lemma}[Informal; Formal version given in \pref{lem:sec-trajectory-convert} in the appendix] Suppose \(\wt \tau'\) denotes a trajectory constructed using \converter{}, and \(\wt \tau\) denotes a trajectory sampled using \(\wtpioff\)  in \(\wt M\). If every \(K\) size buffer in \(\wt \tau'\) has at least some action that deviates from \(\pieval\), then the distribution of \(\wt \tau'\) is identical to that of \(\wt \tau\). 
\end{lemma} 
Furthermore, the buffer-gadget ensures that: 
\begin{lemma}[Informal; Formal version in \pref{lem:sec-trajectory-concentrability} in the appendix] \label{lem: preserve concentrability in convert}  For all \(h \leq H\), the concentrability coefficient   
$\nrm*{\nicefrac{d_h^{\wtpieval}}{d_h^{\wtpiexp}}}_\infty \leq  2\nrm*{\nicefrac{d_h^{\pieval}}{d_h^\piexp}}_\infty$. 
\end{lemma}






The next lemma suggests that estimating the value of \(\wtpieval\) in \(\wt M\) allows us to estimate the value of \(\pieval\) in \(M\).

\begin{lemma}[Informal; Formal version given in \pref{lem:sec-trajectory-equal} in the appendix] Under the lifting operations defined above using the \Replicator-gadget, we have that 
    \begin{align} 
    \wt V^{\wtpieval}(\wt M) = V^{\pieval}(M),  
    \end{align} 
    where  \(V^{\pieval}(M)\) is the value of the policy \(\pieval\) in \(M\) and \(\wt V^{\wtpieval}(\wt M)\) is the value of the policy \(\wtpieval\) in \(\wt M\). 
\end{lemma}


%\begin{algorithm}
%    \caption{Reduction of Offline RL from Admissible Data to Trajectory Data} 
%    \label{alg:convert-admissible} 
%    \begin{algorithmic} 
%        \KwData{For each $h \in [H]$, admissible dataset $\Da_h$ size $Kn$.}
%        \KwData{$Q$-function together with $\mu Q$-function class $\mathcal{F}$ (see \pref{lem:sec-trajectory-equal} for the definition).}
%        \KwData{Offline Algorithm $\At$ that takes trajectory data and $Q$ function class as input and returns a value estimation.}
%        
%        \KwResult{Initialize $\Dt = \emptyset$.}
%        
%        \For{$j = 1, \dots, n$}{
%            \For{$h \in [K]$}{
%                \State Construct $\cD^{\textsc{adm}, j}_h = \Da_h[K(j-1) + 1: Kj]$
%            }
%            \State Get trajectory $\tau^j = \converter(\cD^{\textsc{adm}, j}_1, \dots, \cD^{\textsc{adm}, j}_H)$.
%            \State Update $\Dt \leftarrow \Dt \cup \{ \tau^j \}$.
%        }
%        
%        \State Construct $Q$-function class $\wt{\mathcal{F}}$ according to \pref{eq:sec-trajectory-Q} based on $\mathcal{F}$.
%        \KwResult{Return $\wh V \leftarrow \At(\Dt, \wt{\mathcal{F}})$.}
%    \end{algorithmic}
%\end{algorithm}

\begin{algorithm}
    \caption{Reduction of Offline RL from Admissible Data to Trajectory Data} 
    \label{alg:convert-admissible} 
    \begin{algorithmic}[1] 
        \Require 
        \item[]  \begin{itemize}
            \item For each \(h \in [H]\), admissible dataset \(\Da_h\) size \(Kn\). 
            \item $Q$-function together with $\mu Q$-function class $\mathcal{F}$ (see \pref{lem:sec-trajectory-equal} for the definition);  
            \item Offline Algorithm \(\At\) that takes trajectory data and $Q$ function class as input and returns a value estimation. 
        \end{itemize}   
        \State Initialize \(\Dt = \emptyset\). 
        \For{$j = 1, \dots, n$}
            \State For \(h \in [K]\), construct \(\cD^{\textsc{adm}, j}_h = \Da_h[K(j-1) + 1: Kj]\) 
            \State Get trajectory \(\tau^j = \converter\prn*{\cD^{\textsc{adm}, j}_1, \dots, \cD^{\textsc{adm}, j}_H}\). 
            \State Update \(\Dt \leftarrow \Dt \cup \crl{\tau^j}\). 
        \EndFor
        \State Construct $Q$-function class $\wt{\mathcal{F}}$ according to \pref{eq:sec-trajectory-Q} based on $\mathcal{F}$.
        \State Return \(\wh V \leftarrow \At(\Dt, \wt{\mathcal{F}})\). 
    \end{algorithmic}
\end{algorithm}


With \converter, we are now able to formally reduce offline RL with admissible data to offline RL with trajectory data.  The reduction is stated in \pref{alg:convert-admissible}.  \pref{alg:convert-admissible} provides a way to solve offline RL with admissible data using an algorithm that handles trajectory data. Furthermore, the trajectory data is synthesized in an \MDP that preserves the concentrability coefficient of the original \MDP (\pref{lem: preserve concentrability in convert}). Overall, if trajectory data with bounded concentrability coefficient is tractable, then so is admissible data by leveraging \pref{alg:convert-admissible}, which contradicts \pref{thm:admissible}. Thus, we conclude that this is not the case. The formal argument of the lower bound and the proof of \pref{thm:trajectory_lower_bound} are provided in \pref{app: proof of reduction}.  


\ascomment{All of the above was copied from the main body and needs to be cleaned up} 

==> files/lower_bound_sketch_old.tex <==
\subsubsection{Why aggregated concentrability? From Tabular MDPs to function approximation} 
\paragraph{Warm up from the tabular setting.} 
To warm up, we show that the concentrability coefficient $\tabC_\epsilon(M, \mu)$ is a sample complexity lower bound for an $\epsilon$-accurate evaluation. 
Below we fix $M, \mu, \epsilon$, and write $\tabC_\epsilon(\pieval, \mu; M)$ simply as $\tabC$. By definition (\pref{sec: concen coeff}), the quantity $\tabC$ ensures that there exists a subset of states $\gI$ such that 1) the total occupancy measure on $\gI$ under $\pieval$ is at least $\epsilon$; 2) the ratio of the occupancy measure between the target policy $\pieval$ and the offline data $\mu$ on the state-action sets $\{(\sx, \pieval(\sx))\}_{\sx\in\gI}$ is $\tabC$. 

To see why $\tabC$ serves as a sample complexity lower bound, we design two reward functions $r\ind{1}, r\ind{2}$ such that $r\ind{1}(\sx, \pieval(\sx))=1$, $r\ind{2}(\sx, \pieval(\sx))=-1$ for all $\sx\in\gI$, and $r\ind{1}(\sx,\sa)=r\ind{2}(\sx,\sa)=0$ for all other state-action pairs. Let the environment uniformly randomly make one of them the true reward function. Since these two reward function differs by $2$ on the set $\{(\sx, \pieval(\sx))\}_{\sx\in\gI}$ and this set has an occupancy measure greater than or equal to $\epsilon$ under $\pieval$, in order to make an $\epsilon$-accurate evaluation for $\pieval$, the learner has to figure out which one is the true reward function (otherwise the expected error would be $\Omega(2\cdot\epsilon)$). However, the only way the learner can tell the difference between the two cases is by visiting $\{(\sx, \pieval(\sx))\}_{\sx\in\gI}$, which requires at least $\frac{1}{\sum_{\sx\in \cI} \mu(\sx, \pieval(\sx))} \geq \tabC$ offline samples in expectation. Notice that to make the problem realizable, we only need to let $\gF=\{Q^\pieval(\cdot,\cdot~;M\ind{1}), Q^\pieval(\cdot,\cdot~; M\ind{2})\}$ where $M\ind{i}$ is $M$ equipped with the reward function $r\ind{i}$. 

\paragraph{What is the best the learner can do for function approximation in a large state space? }
Next, we provide some intuition on why the aggregated concentrability serves as a lower bound for policy evaluation in large state spaces. 
In this regime, previous works by \cite{xie2021batch} and \cite{foster2022offline} have already hinted that the difficulty comes from the hardness to distinguish states that have different transition behaviors but the same values. 
Recall that every piece of data is of the form $(\sx, \sa, \sr, \sx')$. If $\sx_1$ and $\sx_2$ are two states appearing in the dataset such that $\gF$ does not provide any information to distinguish them, i.e., $f(\sx_1, \cdot)=f(\sx_2, \cdot)$ for all $f\in\gF$, then the learner has no clue from $\gF$ whether they are essentially the same state or not \asedit{from the perspective of MDP dynamics} \ascomment{How about if I say "whether they inform different feedback about the MDP"}. 
There are also no clues from other parts of the dataset, since with high probability, every state only appears at most once in the dataset due to the large state space. Under such a challenging scenario, the learner almost can do nothing but to \emph{aggregate} these two states, which essentially treats them as the same state, to get the most out of the dataset and the function set. 

The aggregation idea is explicitly used by the algorithm of \cite{xie2021bellman}. When $\gF=\{f\ind{1}, f\ind{2}\}$, their algorithm aggregates state-actions with the same $(f\ind{1}(\sx,\sa), f\ind{2}(\sx,\sa))$ value, and performs empirical Bellman error minimization on this aggregated MDP. In this way, the problem essentially becomes a tabular one on the aggregated state space. Then according to the warm-up discussion, the sample complexity lower bound is governed by the concentrability coefficient --- but now, this concentrability coefficient is defined on the \emph{aggregated} MDP rather than in the original MDP. In \pref{sec: general lower bound sketch}, we provide a proof sketch that formalize this intuition, demonstrating that the aggregation approach by \cite{xie2021bellman} is exactly the \emph{best the learner can do}. 


\subsubsection{Lower bound construction and proof sketch } \label{sec: general lower bound sketch} 
Suppose we are given an arbitrary MDP structure $M$ (without reward function) with state space $\gZ$, any data distribution $\mu$, and any state aggregation scheme $\Phi$ as shown in  \pref{fig: original M}. For simplicity, below we assume that the action set $\gA$ contains an action $\sa_1$, and $\pieval(\sz)=\sa_1$ for all $\sz$. Let $T(\sz'\mid \sz, \sa)$ denote the transition in $M$. In \pref{fig: lower bound general}, states are represented with circles and state aggregations are represented with rectangles. We use the bold rectangle to denote the set of  aggregations $\gI$ that attains the maximum in the definition of $\aggC_\epsilon(M,\Phi,\mu)$ (see \pref{def:agg-concentrability}). Notice that $\gI$ may contain multiple aggregations in general, though in the example of \pref{fig: original M} it contains a single aggregation which contains a single state $\sz^\star$. Also, we assume $\gI$ is in layer $H$ without loss of generality. Below, based on $M$, we will construct two MDPs $M\ind{1}$ (with transitions $T\ind{1}$ and reward $r\ind{1}$) and $M\ind{2}$ (with transitions $T\ind{2}$ and reward $r\ind{2}$). We will argue that it is difficult for the learner to tell them apart when the MDPs are lifted to \emph{block MDPs} (in the Step~6 below we will explain the lifting). 

\begin{figure}[t]
\begin{center}
\subfigure[Original MDP $M$ and aggregation scheme $\Phi$.]{\includegraphics[width=0.385\linewidth]{figures/originalM2.png} \label{fig: original M}}
\hfill  \subfigure[Augmented MDP $M'$ and aggregation scheme $\Phi'$.]{\includegraphics[width=0.465\linewidth]{figures/modifiedM2.png} \label{fig: modified M} } \\ \vspace{50pt}  

\subfigure[Determine the last-layer reward and value functions. \textcolor{red}{Put dots before to signify that this is in the last layer}]{\includegraphics[width=0.37\linewidth]{figures/lastlayer2.png} \label{fig: last layer}}  
\hfill  \subfigure[Determine the value functions inductively.]{\includegraphics[width=0.33\linewidth]{figures/back-propagate2.png} \label{fig: back prob} } \\

\caption{Lower bound construction for general data. \textcolor{red}{Should we write \(h = 1, \dots\) in the above to discuss layering w.r.t.~\(h\)?} } \label{fig: lower bound general} 
\end{center}
\end{figure}

% \begin{figure}[t]
%    %\hspace*{5pt}
%    \hfill
%         \includegraphics[width=0.66\linewidth]{figures/back-propagate2.png}
%         \vspace*{10pt}
%         \caption{Determine the value functions inductively. } \label{fig: back prob}
%     \end{subfigure}%
%     \caption{Lower bound construction for general data. } \label{fig: lower bound general}
% \end{figure} 

%\begin{figure}[t]
%    %\hspace*{5pt}
%    \begin{subfigure}{0.5\textwidth}
%        \centering
%        \includegraphics[width=0.77\linewidth]{figures/originalM2.png}
%        \vspace*{10pt}
%        \caption{Original MDP $M$ and aggregation scheme $\Phi$.}
%        \label{fig: original M}
%    \end{subfigure}% 
%    \hfill
%    \begin{subfigure}{0.5\textwidth}
%        \centering
%        \includegraphics[width=0.93\linewidth]{figures/modifiedM2.png}
%        \vspace*{10pt}
%        \caption{Augmented MDP $M'$ and aggregation scheme $\Phi'$.}
%          \label{fig: modified M}
%     \end{subfigure}\\[1.4cm]
%     \begin{subfigure}{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.74\linewidth]{figures/lastlayer2.png}
%         \vspace*{10pt}
%         \caption{Determine the last-layer reward and value functions. } \label{fig: last layer}
%     \end{subfigure}%
%     \begin{subfigure}{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.66\linewidth]{figures/back-propagate2.png}
%         \vspace*{10pt}
%         \caption{Determine the value functions inductively. } \label{fig: back prob}
%     \end{subfigure}%
%     \caption{Lower bound construction for general data. } \label{fig: lower bound general}
% \end{figure} 


\begin{enumerate}
    \item Construct a modified structure $M'$ with state space $\gZ'$ by augmenting the state space of $M$ with three additional states $\su_h, \sv_h, \sw_h$ on each layer (\pref{fig: modified M}). Let each of $\su_h, \sv_h, \sw_h$ forms an aggregation by itself. %For simplicity, here we assume $\su_h$ and $\sv_h$ are \emph{terminal} states, meaning that when after transitioning to any of them, the episode ends. This slightly violates our fixed-horizon setting, but can be easily addressed by introducing an additional dummy state, which will be handled in our formal proof. 
    Every $\su_h$ has a deterministic reward of $1$ (no matter what action is taken), every $\sv_h$ has a deterministic reward of $-1$, and every $\sw_h$ has a deterministic reward of $0$. All $\su_h$, $\sv_h$, and $\sw_h$ transition to $\sw_{h+1}$ with probability one under any action, and $\sw_{h+1}$ can only be transitioned to from $\su_h$, $\sv_h$, and $\sw_h$. 

    \item Furthermore, for a transition $T(\sz'\mid \sz, \sa)$ in the original MDP $M$, scale its value down by a factor $(1-\frac{1}{H})$ in the modified MDP $M'$ as indicated in \pref{fig: modified M}. This implies that from any state in $\gZ_h$ (i.e., the $h$-th layer in the original MDP $M$), the probabilities of transitioning to $\su_{h+1}$ and $\sv_{h+1}$ need to sum to $\frac{1}{H}$. 
    Up to this point, the modified structure $M'$ is a backbone shared by $M\ind{1}$ and $M\ind{2}$. The transition probabilities from $\gZ$ to $\{\su_h, \sv_h\}_{h=1}^H$ will differ in $M\ind{1}$ and $M\ind{2}$, which will be determined later jointly with reward/value functions (Step~5). 
    \item To ensure concentrability in the modified structure $M'$, on layer $h$, we let $\mu_h'(\sz, \sa) = (1-\frac{1}{H})^{h-1}\mu_h(\sz, \sa)$ for $\sz\neq \su_h, \sv_h, \sw_h$. Notice that the factor $(1-\frac{1}{H})^{h-1}$ is exactly how much the occupancy on $\sz$ (of any policy) is scaled down in $M'$ according to the definition of transition probabilities in Step 2. The modified occupancy on the augmented states $\mu_h'(\su_h, \sa), \mu_h'(\sv_h, \sa), \mu_h'(\sw_h, \sa)$ are defined naturally according to their occupancy in the modified MDP, i.e., define $\mu_h'(\mathsf{s}, \sa) = d_h^{\pieval}(\mathsf{s}, \sa; M')$ for $\mathsf{s} = \su_h, \sv_h, \sw_h$. This way, we can ensure that $\tabC$ (and $\aggC$) remain the same in the original $M$ and in the modified $M'$.
    %\item Create two MDPs $M_1'$ and $M_2'$, each of which is similar to $M$ but has two additional states $\su_h, \sv_h$ on each layer $h\geq 2$. The structures of $M_1'$ and $M_2'$ are almost identical and both inherit from that of $M$. They only differ in the transition probabilities to $\su_h$, $\sv_h$ (the transition probabilities to $\su_h$, $\sv_h$ will be determined jointly with the $r_1, r_2$ in the Step~3 below). 
    %\item Augment $\Phi$ by letting $\su_h$ and $\sv_h$ be two additional aggregations on their own. Call this new aggregation scheme $\Phi'$ ($\Phi'$ is shared by $M_1'$ and $M_2'$). Therefore, 
%$|\Phi_h'|=|\Phi_h|+2$ for $h\geq 2$.  Augment $\mu$ by incorporating some trivial data on states $\su_h, \sv_h$. Call this new data distirbution $\mu'$ (again, shared by $M_1'$ and $M_2'$).  
    \item Create two reward functions $r\ind{1}$ and $r\ind{2}$ on the structure $M'$. For states in 
    $\gI$, let $r\ind{1}(\sz, \pieval(\sz))=\frac{1}{2H}$ and $r\ind{2}(\sz, \pieval(\sz))=-\frac{1}{2H}$; for all other state-actions except for $\{\su_h, \sv_h, \sw_h\}_{h\in[H]}\times \gA$, let $r\ind{1}(\sz, \sa)=r\ind{2}(\sz, \sa)=0$ (\pref{fig: last layer}). 
    \item \textbf{(Key Step)} The key step is to inductively determine the value functions  
$Q\ind{1}(\sz, \sa), Q\ind{2}(\sz, \sa)$ for all $(\sz, \sa)\in\gZ\times \gA$ and the transition probabilities to $\su_h$ and~$\sv_h$, trying to make the learner unable to distinguish the two MDPs. Suppose that all value functions $Q\ind{i}(\sz, \sa)$ are already determined for all $\sz\in \gZ_{h+1}\cup \cdots \cup \gZ_H$, and now we would like to determine the value $Q\ind{i}(\sz, \sa)$ as well as the transition probabilities $T\ind{i}(\su_{h+1}\mid \sz, \sa)$ and $T\ind{i}(\su_{h+1}\mid \sz, \sa)$ for all $\sz\in\gZ_h$. 
    
   We focus on determining these values for the states in the aggregation $\phi$ indicated in \pref{fig: back prob}.  There are two criteria that we would like to satisfy. First, for all states in $\phi$, we would like their state values to be the same in both $M\ind{1}$ and $M\ind{2}$. That is, for any $\sx, \sy\in\phi$ and all $\sa$, we want $Q\ind{1}(\sx, \sa) = Q\ind{1}(\sy, \sa)$ and $Q\ind{2}(\sx, \sa) = Q\ind{2}(\sy, \sa)$. By making so, the learner cannot distinguish the states in the same $\phi$ by looking at the function set $\gF=\{Q\ind{1}, Q\ind{2}\}$. This is the exact reason why we would like to add $\su_{h+1}$ and $\sv_{h+1}$ --- %with only the original transition in $M$, the states in $\phi$ may have different values; however, 
    by splitting out some transition probabilities to $\su_{h+1}$ and $\sv_{h+1}$, and adjust their differences properly (notice that $Q\ind{i}(\su_{h+1}, \sa)=1$ and $Q\ind{i}(\sv_{h+1}, \sa)=-1$), we can calibrate the state-action values in $\phi$, making them all equal. This criteria can be formally expressed as 
    \begin{align}
    &\forall i=1,2,\quad \forall \sz\in \phi, \quad \forall \sa\in \gA, \nonumber \\
    &\quad  \sum_{\sz'\in \gZ_{h+1}}  T'(\sz'\mid \sz, \sa) V\ind{i}(\sz') + T\ind{i}(\su_{h+1}\mid \sz, \sa) \cdot 1 +  T\ind{i}(\sv_{h+1}\mid \sz, \sa)\cdot(-1) = Q\ind{i}(\phi, \sa).    \label{eq: criteria1}
\end{align}
    The left-hand side is the expression of $Q\ind{i}(\sz, \sa)$, where $V\ind{i}(\sz')\ldef{}  Q\ind{i}(\sz', \pieval(\sz'))=Q\ind{i}(\sz', \sa_1)$. On the right-hand side we abuse the notation $Q\ind{i}(\phi, \sa)$ to indicate that this is value of $Q\ind{i}(\sz, \sa)$ shared by all states $\sz\in \phi$. 
    %Notice that in the two MDPs $i=1,2$, the transition probabilities to $\su_{h+1}$ (or $\sv_{h+1}$) need to be different because in general $V\ind{1}(\sz')\neq V\ind{2}(\sz')$ for $\sz'\in\gZ_{h+1}$. 
    
    The second criteria is to make the learner unable to tell the difference between the two MDPs by looking at the transitions to $\su_{h+1}$ and $\sv_{h+1}$. Since we have already made the learner unable to distinguish states in the same $\phi$ (Technically, we need to create rich observation copies of each state to rigorously argue that the learner cannot tell them apart. See Step~6), it suffices to make sure that the \emph{aggregated} transition (over states in $\phi$) to $\su_{h+1}$ and $\sv_{h+1}$ is indistinguishable between the two MDPs. Formally, the second criteria can be expressed as 
    \begin{align}
         &\forall \sa\in \gA, \quad \sum_{\sz\in\phi}\mu_h(\sz, \sa) T\ind{1}(\su_{h+1}\mid \sz, \sa) = \sum_{\sz\in\phi}\mu_h(\sz, \sa) T\ind{2}(\su_{h+1}\mid \sz, \sa), \nonumber  \\
         &\forall \sa\in \gA, \quad  \sum_{\sz\in\phi}\mu_h(\sz, \sa) T\ind{1}(\sv_{h+1}\mid \sz, \sa) = \sum_{\sz\in\phi}\mu_h(\sz, \sa) T\ind{2}(\sv_{h+1}\mid \sz, \sa),   \label{eq: indistinguishable}
    \end{align}
    where the first line is the overall transition from $(\phi,\sa)$ to $\su_{h+1}$ seen by the learner, and the second is the overall transition from $(\phi, \sa)$ to $\sv_{h+1}$. %That is, although $T\ind{1}(\su_{h+1}\mid \sz, \sa)\neq T\ind{2}(\su_{h+1}\mid \sz, \sa)$ in general (or $\sv_{h+1}$), we make the aggregated transition over $\phi$ the same for $i=1$ and~$2$. 
    
   One can show that there exist solutions for $(Q\ind{i}(\sz, \sa)$, $T\ind{i}(\su_{h+1}\mid \sz, \sa), T\ind{i}(\sv_{h+1}\mid \sz, \sa))_{i\in[2], \sz\in\phi, \sa\in \gA}$ that satisfy \pref{eq: criteria1} and \pref{eq: indistinguishable} and the constraint $T\ind{i}(\su_{h+1}\mid \sz, \sa) + T\ind{i}(\sv_{h+1}\mid \sz, \sa)=\frac{1}{H}$ mentioned in Step~2. In fact, one solution is given by (see \pref{lem:sec-lower-bound-latent-MDP} for a derivation)
   \begin{align}
       Q\ind{i}(\phi, \sa) = \sum_{\phi'\in \Phi_{h+1}} \agg{T}(\phi'\mid \phi, \sa) V\ind{i}(\phi'),  \label{eq: natural sol} %\\
       %\forall \sz\in\phi, \forall \sa\in\gA,  
 %&\quad  T\ind{i}(\su_{h+1}\mid \sz, \sa)  -  T\ind{i}(\sv_{h+1}\mid \sz, \sa) = Q\ind{i}(\phi, \sa) -  \sum_{\sz'\in \gZ_{h+1}}  T'(\sz'\mid \sz, \sa) V\ind{i}(\sz'),     \label{eq: calibrate}  \\
         %\forall \sz\in\phi, \forall \sa\in\gA, 
%&\quad T\ind{i}(\su_{h+1}\mid \sz, \sa) +  T\ind{i}(\sv_{h+1}\mid \sz, \sa) = \frac{1}{H}. 
 %\label{eq: sum constraint} 
   \end{align}
   where $\Phi_{h+1}$ is the set of aggregations on layer $h+1$ excluding $\su_{h+1}, \sv_{h+1}, \sw_{h+1}$, $\agg{T}(\phi'\mid \phi, \sa) = \frac{\sum_{\sz'\in\phi'}\sum_{\sz\in\phi} \mu_{h}(\sz, \sa) T'(\sz'\mid \sz, \sa)}{\sum_{\sz\in\phi} \mu_{h}(\sz, \sa) }$ is the aggregated transition, and $V\ind{i}(\phi')\ldef{}  Q\ind{i}(\phi', \sa_1)$. The values of $T\ind{i}(\su_{h+1}\mid \sz, \sa)$ and $T\ind{i}(\sv_{h+1}\mid \sz, \sa)$ can be obtained by plugging \pref{eq: natural sol} into \pref{eq: criteria1} (which gives the value of $T\ind{i}(\su_{h+1}\mid \sz, \sa)-T\ind{i}(\sv_{h+1}\mid \sz, \sa)$) and solving it jointly with $T\ind{i}(\su_{h+1}\mid \sz, \sa)+T\ind{i}(\sv_{h+1}\mid \sz, \sa)=\frac{1}{H}$. 
  
  \iffalse
  With \pref{eq: natural sol}, we can obtain the values of $T\ind{i}(\su_{h+1}\mid \sz, \sa)$ and $T\ind{i}(\sv_{h+1}\mid \sz, \sa)$ by plugging \pref{eq: natural sol} into \pref{eq: criteria1} (which gives the value of $T\ind{i}(\su_{h+1}\mid \sz, \sa)-T\ind{i}(\sv_{h+1}\mid \sz, \sa)$) and solving it jointly with $T\ind{i}(\su_{h+1}\mid \sz, \sa)+T\ind{i}(\sv_{h+1}\mid \sz, \sa)=\frac{1}{H}$. 
  

   %To get more sense about this solution, note that when \pref{eq: criteria1} is combined with \pref{eq: natural sol}, we obtain 
   %\begin{align}
   %    T\ind{i}(\su_{h+1}\mid \sz, \sa)  -  T\ind{i}(\sv_{h+1}\mid \sz, \sa) = \sum_{\phi'\in \Phi_{h+1}} \agg{T}(\phi'\mid \phi, \sa) V\ind{i}(\phi') -  \sum_{\sz'\in \gZ_{h+1}}  T'(\sz'\mid \sz, \sa) V\ind{i}(\sz').    \label{eq: calibrate}
   %\end{align}
   %That is, the transition difference $T\ind{i}(\su_{h+1}\mid \sz, \sa)  -  T\ind{i}(\sv_{h+1}\mid \sz, \sa)$ is going to calibrate the original value $\sum_{\sz'\in \gZ_{h+1}}  T'(\sz'\mid \sz, \sa) V\ind{i}(\sz')$ to $\sum_{\phi'\in \Phi_{h+1}} \agg{T}(\phi'\mid \phi, \sa) V\ind{i}(\phi')$, which is equalized among $\sz\in\phi$. %Combining this with the condition $T\ind{i}(\su_{h+1}\mid \sz, \sa) + T\ind{i}(\sv_{h+1}\mid \sz, \sa)=\frac{1}{H}$, we can obtain individual values of $T\ind{i}(\su_{h+1}\mid \sz, \sa) $ and $T\ind{i}(\sv_{h+1}\mid \sz, \sa)$ (it is easy to argue that they are non-negative). 
   
   %To see the $Q\ind{i}(\phi, \sa)$ in \pref{eq: natural sol} gives a feasible solution, notice that when \pref{eq: criteria1} is combined with \pref{eq: natural sol}, we obtain the values of $T\ind{i}(\su_{h+1}\mid \sz, \sa) - T\ind{i}(\sv_{h+1}\mid \sz, \sa)$ for all $(\sz, \sa)\in\phi\times \gA$. Further combining this with the condition $T\ind{i}(\su_{h+1}\mid \sz, \sa) + T\ind{i}(\sv_{h+1}\mid \sz, \sa)=\frac{1}{H}$, we obtain individual values of $T\ind{i}(\su_{h+1}\mid \sz, \sa) $ and $T\ind{i}(\sv_{h+1}\mid \sz, \sa)$ (it is easy to argue that they are both non-negative). It remains to verify that the solution obtained in this way satisfies \pref{eq: indistinguishable}. 
   To verify that the solution obtained above satisfies \pref{eq: indistinguishable}, observe that
   \begin{align*}
      &\sum_{\sz\in\phi} \mu_h(\sz, \sa) \left(T\ind{i}(\su_{h+1}\mid \sz, \sa) - T\ind{i}(\sv_{h+1}\mid \sz, \sa)\right) \\
      &= \sum_{\sz\in\phi} \mu_h(\sz, \sa) \left(Q\ind{i}(\phi, \sa) - \sum_{\sz'\in\gZ_{h+1}} T'(\sz'\mid\sz, \sa) V\ind{i}(\sz')\right)   \tag{by \pref{eq: criteria1}} \\
      &= \sum_{\sz\in\phi} \mu_h(\sz, \sa) \left(\sum_{\phi'\in\Phi_{h+1}}\frac{\sum_{\sz'\in\phi'}\sum_{\tilde{\sz}\in\phi} \mu_h(\tilde{\sz}, \sa)T'(\sz'\mid\tilde{\sz}, \sa) }{\sum_{\tilde{\sz}\in\phi}  \mu_h(\tilde{\sz}, \sa)}V\ind{i}(\phi') - \sum_{\sz'\in\gZ_{h+1}} T'(\sz'\mid\sz, \sa) V\ind{i}(\sz')\right)   \tag{by \pref{eq: natural sol} and the definition of $\agg{T}(\phi'\mid\phi, \sa)$ } \\
      &=\sum_{\tilde{\sz}\in\phi} \mu_h(\tilde{\sz}, \sa)\sum_{\sz'\in\gZ_{h+1}} T'(\sz'\mid\tilde{\sz}, \sa) V\ind{i}(\sz') - \sum_{\sz\in\phi} \mu_h(\sz, \sa)\sum_{\sz'\in\gZ_{h+1}} T'(\sz'\mid \sz, \sa) V\ind{i}(\sz')= 0. 
   \end{align*}
   That is, the aggregated transition to $\su_{h+1}$ and to $\sv_{h+1}$ are the same. Combining this with $T\ind{i}(\su_{h+1}\mid \sz, \sa) + T\ind{i}(\sv_{h+1}\mid \sz, \sa) =\frac{1}{H}$, we get $\sum_{\sz\in\phi} \mu_h(\sz, \sa) T\ind{i}(\su_{h+1}\mid \sz, \sa) = \sum_{\sz\in\phi} \mu_h(\sz, \sa) T\ind{i}(\sv_{h+1}\mid \sz, \sa) = \frac{1}{2H}\sum_{\sz\in\phi}\mu_h(\sz, \sa)$ for both $i=1,2$, which verifies \pref{eq: indistinguishable}. 

    
   %Importantly, \pref{eq: natural sol} indicates that $Q\ind{i}(\phi, \sa)$ follows the Bellman equation with $\agg{T}$ as the transition and $\Phi$ as the state space. 

    Overall, there exist solutions of $(Q\ind{i}(\sz, \sa)$, $T\ind{i}(\su_{h+1}\mid \sz, \sa), T\ind{i}(\sv_{h+1}\mid \sz, \sa))$ for all $\sz\in\gZ_h$, $\sa\in\gA$ and $i=1,2$ so that the two criteria are satisfied simultaneously.  The procedure above are repeated for $h=H-1, H-2, \ldots, 1$. 
    \fi

    \item We remark that although in Step~5 we have assigned the same value of $(Q\ind{1}(\sz, \cdot), Q\ind{2}(\sz, \cdot))$ to all states $\sz$ within the same aggregation, this alone does not prevent the learner from differentiating the states. If those states appear multiple times in the dataset, the learner might still tell them apart by distinguishing the their transition behaviors. To eliminate the possibility of this, we lift $M\ind{1}$ and $M\ind{2}$ to block MDPs where every state $\sz$ serves as a \emph{latent state} invisible to the learner. Instead of observing the latent state $\sz$, the learner only observes a \emph{rich observation} associated with~$\sz$. This conceals the real identity of $\sz$ from the learner, and leaves $(Q\ind{1}(\sz, \cdot), Q\ind{2}(\sz, \cdot))$ as the only information the learner can leverage to distinguish states. %We can make the rich observation space large enough so that with high probability there are no repeated rich observations appearing in the dataset. %Since the value of  $(Q\ind{1}(\sz, \cdot), Q\ind{2}(\sz, \cdot))$ is the same for all $\sz$'s within the same aggregation $\phi$, it does not provide information on the identity of the state. 
    %Thus, unless there are repeated rich observations in the dataset (which is very unlikely if we make the rich observation space very large), there is no way for the learner to discern transition behavior on individual latent states within the same aggregation.  
    This solidifies our argument made in Step~5. %: by lifting the models to block MDPs and equating the value functions for all states in the same aggregation, the individual identities of states within the same aggregation are concealed. 
    The technique we use here is similar to that used by \cite{foster2022offline}. 
    %Furthermore, given the large size of the rich observation space, each observation is likely to occur only once within the dataset, making it difficult for the learner to learn the transition behavior on individual states. The best the learner can do is to learn the \emph{aggregated} transition behavior, with the resolution provided by $(Q\ind{1}(\cdot, \sa), Q\ind{2}(\cdot, \sa))$.  which is the same for two rich observations in the same aggregation. 

    \item Notice that the $Q\ind{i}$ in \pref{eq: natural sol} satisfies a Bellman equation under the aggregated transition $\agg{T}$. By the same argument as in the tabular warm-up, it is straightforward to verify that a difference of $|Q\ind{1}(\sz^\star, \pieval(\sz^\star)) - Q\ind{2}(\sz^\star, \pieval(\sz^\star))|=\frac{1}{H}$ leads to a difference of  $|\E_{\sz\sim \rho}V\ind{1}(\sz) - \E_{\sz\sim \rho}V\ind{2}(\sz)|=\frac{1}{H}\cdot \agg{d}(\sz^\star)\geq \Omega(\epsilon/H)$ on the initial state, where $\agg{d}(\sz^\star)$ is the occupancy measure of $\sz^\star$ under the transition $\agg{T}(\sz'\mid\sz, \sa)$. By our construction in Step~5 and Step~6, the learner cannot obtain useful information by visiting states other than $\sz^\star$. Thus, the only way the learner can tell the two environments apart is by visiting $\sz^\star$, which requires at least $\Omega(\frac{1}{\mu(\sz^\star, \pieval(\sz^\star))})\geq \Omega(\aggC)$ samples.   
    %respectively, so that states in the same aggregation always share their value functions (i.e., $f_1(\sx, \cdot)=f_1(\sx', \cdot)$ and $f_2(\sx, \cdot)=f_2(\sx', \cdot)$ if $\sx$ and $\sx'$ belong to the same aggregation under $\Phi'$). 
    %\item Create two \emph{classes} of MDPs $\gM_1$ and $\gM_2$. Each MDP in $\gM_i$ is essential a rich observation 
    %representation of a block MDP with $M_i'$ as the underlying latent MDP. 
    %\item Let the true MDP be chosen uniformly from $\gM_1\cup \gM_2$. Argue that in order to determine the value of $\pieval$ in the true MDP, the sample complexity is at least $\aggC_\epsilon(M; \Phi, \mu)$.  
\end{enumerate}
In the formal proof, in order to improve the lower bound from 
$\Omega(\aggC)$ to $\Omega(\frac{\aggC}{\epsilon})$, we use randomized reward on $\gI$ instead of deterministic one. The formal proof can be found in \pref{app:proof1}.



==> files/main_agnostic.tex <==
\section{Role of Realizable Value Function Class}  
Can discuss known upper bounds for Agnostic RL. 

\subsection{Small Horizon with \admissible{} Data}

\begin{theorem} \(H=2\), admissible data does not suffice without the function class.  
\end{theorem}

\subsection{Large Horizon with Trajectory Data} 
\begin{theorem} Trajectory data does not suffice without the function class but has strong coverage. 
\end{theorem}


==> files/main_intro_old.tex <==
\section{Introduction}


Offline reinforcement learning (RL) is an RL paradigm where the goal is to either find the optimal policy or evaluate a given policy based solely on pre-collected data (i.e., offline data), without direct interaction with the environment. This paradigm is particularly relevant in situations where real-time interaction is infeasible or expensive, e.g., in safety-critical applications such as healthcare and autonomous driving. The primary challenge in offline RL comes from the mismatch between the offline data distribution and the distribution induced by the target policy (i.e., the optimal policy or the policy to be evaluated), which can severely affect the efficacy of the output policy or evaluation. Therefore, a significant portion of offline RL research is dedicated to mitigating the impact of this mismatch.

Perhaps the most straightforward way to deal with the mismatch is by \emph{importance weighting}. For a trajectory in the offline dataset generated by a behavior policy, its importance weight is the ratio between the probability of this trajectory being generated by the target policy, and probability of it being generated by the behavior policy. This importance weight can be exponential in the trajectory length even when the target policy and the behavior policy's probability of choosing every action is bounded by a constant. This leads to exponentially large sample variance and potentially bad sample efficiency. 

To address this issue, researchers resort to approaches that exploit the Markov property of the environment and use function approximation to generalize across states. One such approach is \emph{model-based approach}, where the learner explicitly models the transition and the reward functions. When model realizability holds, the dependence on the importance weight can be reduced to the \emph{concentrability coefficient}, defined as the largest ratio between the probability of a state-action pair being visited by the target policy and the frequency of it in the offline data (formally defined in \pref{sec: concen coeff}). The concentrability coefficient always lower bounds the maximum possible importance weight.  However, model-based approaches also introduce a dependence on the complexity of the model class. For example, in a finite model class $\gM$, the worst-case complexity is $\log|\gM|$, which could be large. 

Another approach is the \emph{value-based approach}, where the learner only approximates the value function of the target policy. Usually, the value function class size could be much smaller than the model class size. However, even when the true value function lies in the function set (i.e., value function realizable setting), all prior work that establish polynomial sample complexity make more assumptions than just bounded concentrability coefficient. As far as we know, such additional assumptions include 1) Bellman completeness \ascomment{need citation!} or $\beta$-incompleteness with $\beta<1$ \citep{zanette2023realizability}, 2) density-ratio realizability \citep{xie2020q}, and 3) pushforward concentrability \citep{xie2021batch}. Any of these conditions along with bounded concentrability can lead to polynomial sample complexity. However, it remained open for a long time whether concentrability alone allows for polynomial sample complexity. 
%To quantify the distribution mismatch between the offline dataset and the target policy, the notion of \emph{concentrability coefficient} has been widely used. The standard concentrability coefficient is defined as the largest ratio in the frequency of a specific state-action pair being visited by the target policy compared to their occurrence in the offline data (formally defined in XXXXXX). 

The work of \cite{foster2022offline} first gave a negative answer to this open problem.  They showed that realizability and concentrability alone cannot ensure polynomial sample complexity. Their lower bound construction, however, rely on the offline data being generated in an unnatural way --- the offline data distribution has to either cover state-actions that will never be visited by any policy, or has to come from just the first two steps in an episode, with all data from later steps hidden from the learner. Thus, the following question remains open: 
\begin{center}
\textit{Is polynomial sample complexity possible under value function realizability and natural offline data distribution, such as trajectories generated by a single behavior policy?} 
\end{center}

Our work provides a negative answer to this question. That is, we show that there exist MDPs where the offline data consists of trajectories generated by a single behavior policy, the value function is realizable by a small function class, and the concentrability coefficient is polynomial in the horizon length, but the sample compelxity is exponential in the horizon length. This formally shows that value function realizability alone does not provide much benefit over importance weighting in terms of sample complexity. Stronger conditions are required to make it efficient.  

To establish this result, we actually provide a rather complete characterization for offline RL with value function realizability. First, we show that in order to achieve sample efficiency, the concept of ``concentrability'' needs be strengthened. More precisely, the minimax sample complexity under value function realizabilty is precisely characterized by the ``aggregated concentrability coefficient'' in an aggregated transition model, where states with indistinguishable value functions are aggregated, and the transition is determined jointly by the aggregation and the offline data distribution (see \pref{sec: general lower bound} for the upper bound and \pref{sec: upper bound} for the lower bound). 
On one hand, the lower bound of \cite{foster2022offline} is a special case of our lower bound where the aggregated concentrability coefficient is infinitely large or exponentially large in the horizon. On the other hand, the upper bound of \cite{xie2021batch}, which uses the pushforward concentrability coefficient to characterize their sample complexity, is covered by our upper bound, as one can show that the aggregated concentrability coefficient is upper bounded by the pushforward concentrability coefficient.  

Having identified that the aggregated concentrability coefficient is the key quantity, we provide in \pref{sec: admissible data} a simple example where the offline data is admissible, the standard concentrability coefficient is $O(H^2)$, but the aggregated concentrability is $\Omega(H2^H)$, where $H$ is the horizon length. Together with the lower bound established in \pref{sec: general lower bound}, this implies that even if the offline data is admissible, it is impossible to achieve a sample complexity that only polynomially depends on the horizon length, the concentrability coefficent, and the logarithmic function size. This strengthens the previous lower bound result of \cite{foster2022offline} by allowing admissible offline data.  

We next provide a generic \emph{reduction} that converts this hard instance for admissible data into a hard instance for trajectory data. We show that under value function realizability, learning any MDP with admissible data is no harder than learning another MDP with trajectory data, where the horizon length augmented to $O(H\ln H)$ and the concentrability is kept as the same order. This is established in \pref{sec: trajectory lower bound}. Combining the results in \pref{sec: general lower bound}--\pref{sec: trajectory lower bound} gives a concrete answer to the main open question left by \cite{foster2022offline}. 
We remark that the notions of \emph{realizability} and \emph{concentrability} adopted in our paper are only with respect to the \emph{target policy}, but not to all possible policies. Namely, we only assume that the function class realizes the value function of the target policy, but not necessary those of other policies. Similarly, we only assume that the state-action occupancy ratio between the target policy
and the offline data is bounded, but not necessary for other policies. Whether trajectory data allows tractable offline RL under all-policy realizability and under all-policy concentrability both remain open. 



==> files/main_intro_old2.tex <==
\section{Introduction}

Offline reinforcement learning (RL) is an RL paradigm where the goal is to either find the optimal policy (policy optimization) or evaluate a given policy (policy evaluation) based solely on pre-collected data (i.e., offline data), without direct interaction with the environment. This paradigm is particularly relevant in situations where real-time interaction is infeasible or expensive, e.g., in safety-critical applications such as healthcare and autonomous driving. The primary challenge in offline RL comes from the mismatch between the offline data distribution and the distribution induced by the target policy (i.e., the optimal policy or the policy to be evaluated), which can severely affect the efficacy of the output policy or evaluation. Therefore, a large portion of offline RL research aims to mitigate the impact of this mismatch. 

To deal with large state spaces in RL, function approximation is used to generalize the learned knowledge across states. One such approach is the \emph{model-based approach}, where the learner explicitly models the transition and the reward functions. Theoretical research for this approach studies the sample complexity under \emph{model realizability}, i.e., assuming that the learner is provided with a model class that includes the true model \citep{uehara2021pessimistic}. In this setting, the minimax sample complexity is polynomial in the \emph{concentrability coefficient} and the complexity of the model class \citep{uehara2021pessimistic}. The concentrability coefficient is defined as the largest ratio between the probability of a state-action pair being visited by the target policy and the frequency of it in the offline data (formally defined in \pref{sec: concen coeff}), which captures the mismatch between the distribution induced by the offline data and the target policy. The model class complexity captures the diversity of the model class. For a finite model class $\gM$, the worst-case model class complexity is $\log|\gM|$. 

Another approach is the \emph{value-based approach}, where the learner only approximates the value function of the target policy. Usually, the value function class complexity is much smaller than the model class complexity, and is sometimes considered as a simpler and more direct approach. However, under \emph{value function realizability}, all prior work that establish polynomial sample complexity make more assumptions than just bounded concentrability coefficient. Such additional assumptions include 1) Bellman completeness \citep{chen2019information} or $\beta$-incompleteness with $\beta<1$ \citep{zanette2023realizability}, 2) density-ratio realizability \citep{xie2020q}, and 3) pushforward concentrability \citep{xie2021batch}. Any of these conditions along with bounded concentrability coefficient can lead to polynomial sample complexity. However, it remained open for a long time whether concentrability alone allows for polynomial sample complexity. 

The work of \cite{foster2022offline} first gave a negative answer to this open problem.  They showed that realizability and concentrability alone cannot ensure polynomial sample complexity. Their lower bound construction, however, relies on the offline data being generated in an unnatural way --- the offline data distribution has to either cover state-actions that will never be visited by any policy, or has to come from just the first two steps in an episode, with all data from later steps hidden from the learner. Thus, the following question remains open: 

%\noindent
%\textbf{(Main question)} \textit{Can offline RL be statistically efficient under value function realizability, bounded concentrability, and natural offline data such as trajectories generated by a single behavior policy? }
\begin{center}
\begin{minipage}{0.95\textwidth}  
\centering  
\textit{Can offline RL be sample efficient under value function realizability, bounded concentrability, and natural offline data distribution such as trajectories generated by a single behavior policy? }
\end{minipage}  
\end{center} 

Our work takes a first step to answering this question for \emph{offline policy evaluation} (OPE), where the goal is to evaluate the expected payoff of a given policy. Our answer is negative.  Specifically, we show that there exist \MDP instances where the offline data consists of \emph{trajectories} generated by a single behavior policy, the value function is realized by a small function class, and the concentrability coefficient is polynomial in the horizon length, but the worst-case sample compelxity for \OPE has to be exponential in the horizon length. 

En route to establishing this result, we provide a rather complete characterization for \OPE with value function realizability. First, we show that in order to achieve sample efficiency, the concept of ``concentrability'' needs to be strengthened. More precisely, the minimax sample complexity under value function realizabilty is precisely characterized by the ``aggregated concentrability coefficient'' in an aggregated transition model. The aggregated transition model is constructed by aggregating states with indistinguishable value functions, and its transition is jointly determined by the aggregation and the offline data distribution. 
On one hand, our lower bound construction generalizes that of \cite{foster2022offline} by providing instance dependent lower bounds applicable to MDPs with different structures; their construction can be viewed as a special case where the aggregated concentrability coefficient is infinitely or exponentially large. On the other hand, our upper bound recovers the notion of pushforward concentrability coefficient used by \cite{xie2021batch} to establish their sample complexity upper bound \srcomment{wording unclear}, as one can show that the aggregated concentrability coefficient is upper bounded by the pushforward concentrability coefficient.  

Having identified the aggregated concentrability coefficient as the key quantity that governs the sample complexity of offline policy evaluation, we provide a simple example where the offline data distribution is admissible (i.e., the offline data distribution equals the occupancy measure of an offline policy), the standard concentrability coefficient is $\order(H^3)$, but the aggregated concentrability is $2^{\Omega(H)}$, where $H$ is the horizon length. Since  aggregated concentrability governs the sample complexity of offline policy evaluation, 
this implies that realizability, concentrability, and admissibility are not sufficient for sample efficient OPE. 

We next provide a generic \emph{reduction} that converts the aforementioned hard instance for admissible data into a hard instance for trajectory data. We show that under value function realizability, performing \OPE with trajectory data is no easier than performing \OPE with admissible data. 
Combining these two pieces of the puzzle, we conclude that realizability, concentrability, and trajectory data do not jointly guarantee sample efficient OPE, thus answering our main question. 

%To quantify the distribution mismatch between the offline dataset and the target policy, the notion of \emph{concentrability coefficient} has been widely used. The standard concentrability coefficient is defined as the largest ratio in the frequency of a specific state-action pair being visited by the target policy compared to their occurrence in the offline data (formally defined in XXXXXX). 


==> files/main_related_works.tex <==
\subsection{Related Works} 
Offline reinforcement learning is challenging due to the lack of direct interaction with the environment. Existing theoretical works that provide polynomial sample complexity guarantees often rely on multiple assumptions to be satisfied simultaneously. Specifically, in the realm of value function approximation, three pivotal assumptions stand out: (value function) realizability, concentrability, and Bellman completeness. For policy evaluation, realizability and concentrability only refer to the target policy, while for policy optimization, these two assumptions can be further categorized into single-policy (i.e., only satisfied for the optimal policy) and all-policy (satisfied for all policies).  

If Bellman completeness holds, either all-policy realizability with single-policy concentrability \citep{xie2021bellman} or single-policy realizability with all-policy concentrability \citep{chen2019information} can guarantee polynomial sample complexity for policy optimization. The Bellman completeness assumption, however, is deemed rather undesirable because it is non-monotone in the function class and thus may be severely violated when a rich function class is used. Several efforts have been made to remove this assumption, though all requiring new assumptions: \cite{xie2021batch} showed that if a stronger version of concentrability, called \emph{pushforward} concentrability, holds, then with only single-policy realizability, polynomial sample complexity can be achieved without Bellman completeness. \cite{xie2020q}, \cite{zhan2022offline}, and \cite{ozdaglar2023revisiting} introduced the notion of \emph{density-ratio realizability} (different from value function realizability), and showed that this along with single-policy realizability and single-policy concentrability ensures polynomial sample complexity. \cite{zanette2023realizability} relaxed Bellman completeness to the notion of \emph{$\beta$-incompleteness} where Bellman completeness corresponds to $\beta=0$. He proved that $\beta<1$ along with realizability and concentrability admits polynomial sample complexity for policy evaluation.  

The question whether realizability and concentrability alone guarantee efficient learning remained open until the work of \cite{foster2022offline}, who provided a negative answer. They gave two examples where polynomial samples is insufficient even with all-policy realizability and all-policy concentrability. Their first  construction relies on a portion of data coming from unreachable states, and the second construction relies on the data being only collected from the first two steps in an episode.  %one is \emph{over-coverage}, where some offline data is supported on unreachable states. This construction relies on the data being \emph{not admissible}. They provided a strengthened construction where the data is \emph{weakly admissible}. This second construction relies on the data being only collected from the first two steps of an episode to hide the information revealed in later steps. 
It was stated as an open problem by \cite{foster2022offline} whether similar lower bounds can hold under the much more benign scenario where the learner can see \emph{trajectories} generated by an offline policy. This is answered in our paper. 

%\CW{Some other related works to be put in the framework: \cite{uehara2023refined}}

There is another line of works showing exponential lower bound / impossibility for linear function approximation, with concentrability replaced by other weaker notions of coverage \citep{wang2020statistical, amortila2020variant, zanette2021exponential}. Their assumptions do not imply concentrability, and thus these works do not resolve the previous open question. More positive results can be found in the literature of \emph{model-based} approaches, for which we refer the reader to \cite{uehara2021pessimistic} and the related works therin. 

In online reinforcement learning, while value function realizability is still a common assumption, Bellman completeness can usually be replaced by some low rank / low eluder dimension structure on the Bellman error or its estimator \citep{du2021bilinear, jin2021bellman}. Under these structural assumptions, concentrability is no longer needed due to the capability of efficient exploration provided by these structures. Recently, \cite{xie2022role} identified a new structural assumption which resembles all-policy concentrability and ensures polynomial sample complexity when combined with Bellman completeness. It is an interesting direction to further unify the common notions used in online and offline reinforcement learning. 

\ascomment{I think we need further discussions on the role of trajectory information outside of Value Function-Based Offline RL, e.g. goal conditioned RL, etc}  \CW{Okay. Do you want to add those? I don't know much about them.}

\ascomment{Other references: \begin{enumerate}
    \item ``Using Trajectory Data to Improve Bayesian Optimization for Reinforcement Learning", \citep{wilson2014using}. 
\end{enumerate}}


%Offline policy evaluation common assumptions: 
%\begin{itemize}
%     \item 1. value realizability 
%     \item 2. Bellman completeness
%     \item 3. concentrability 
%     \item 4. weight ratio realizability (stronger than 3)
%     \item 5. model realizability
%\end{itemize}
%\begin{itemize}
%    \item 1+2+3: \cite{xie2021bellman}, \cite{chen2019information}
%    \item 1+3: \cite{xie2021batch}, \cite{zanette2023realizability}
%    \item 1+4: \cite{zhan2022offline}, \cite{ozdaglar2023revisiting}
%    \item ... + 5: some paper from Wen Sun
%\end{itemize}
%For offline policy optimization, there's further distinction between all-policy and single-policy value realizability/concentrability.  

%Online policy optimization: 
%\begin{itemize}
%    \item 1. value realizability 
%    \item 2. Bellman completeness
%    \item 3. Bellman rank / bilinear rank / Bellmen eluder
%    \item 4. coverage (somewhat related to concentrability?)
%\end{itemize}

==> files/main_trajectory_data.tex <==
\section{files/main_trajectory_data.tex}
\begin{enumerate}
    \item Difference between \admissible{} and trajectory data. 
    \item Why the previous construction breaks. 
    \item New fix: mimicking strongly admissible data with trajectory data. 
\end{enumerate}

\begin{theorem}\label{thm:trajectory_lower_bound} Exponential lower bound with trajectory data
\end{theorem}

% \begin{theorem} 
%     General result for trajectory data? (may just say in words instead of a formal theorem)
% \end{theorem}



==> files/old_lb_proof.tex <==
69\begin{lemma}
    Suppose for every $\phi\in \Psi$, we have 
    $$|\calX(\phi)|\ge \frac{32|\phi|^4H^3\ophatC{M}{\mu}{\epsilon}{\Phi}^3}{\epsilon^3}.$$
    If $n\le \frac{H}{8\epsilon} \ophatC{M}{\mu}{\epsilon}{\Phi}$, then we have
    $$D_{\mathrm{TV}}(\mathbb{P}_n\ind{1}, \mathbb{P}_n\ind{2})\le \frac{1}{2}.$$
\end{lemma}

\begin{proof}
    First of all, we will construct a distribution $\mathbb{P}_n\ind{0}\in\Delta((\cX\times\cA\times \{-1, 1\}\times \cX)^n)$, and according to Triangle inequality we have
    $$D_{\mathrm{TV}}(\mathbb{P}_n\ind{1}, \mathbb{P}_n\ind{2})\le D_{\mathrm{TV}}(\mathbb{P}_n\ind{1}, \mathbb{P}_n\ind{0}) +  D_{\mathrm{TV}}(\mathbb{P}_n\ind{0}, \mathbb{P}_n\ind{2}).$$
    
    To be specific, we define $\mathbb{P}_n\ind{0} = (\mathbb{P}\ind{0})^{\otimes n}$, where $\mathbb{P}\ind{0}$ is defined as
    $$\mathbb{P}\ind{0}((\sx,\sa, r, \sx')) \triangleq \nu(\sx, \sa, \sx')\rich{R}\ind{0}(r\mid \sx, \sa),$$
    where for $\sx\in \calX(\phi)$ and $\sx'\in\calX(\phi')$,
    %\ayush{Why is the following a nicefrak in displayed equation?} 
    \begin{equation}\label{eq:sec-lower-bound-def-nu}
        \nu(\sx, \sa, \sx') = \sum_{\sz\in\phi}\sum_{\sz'\in\phi'} \frac{\mu(\sz, \sa)T\ind{1}(\sz'\mid \sz, \sa)|\phi||\phi'|}{|\calX(\phi)||\calX(\phi')|}
    \end{equation}
    and,
    $$\rich{R}\ind{0}(\cdot \mid \sx,\sa) = \begin{cases}
        \delta(1) &\quad \sx = \su_h,\\
        \delta(-1) &\quad \sx = \sv_h,\\
        \frac{1}{2}\delta(1) + \frac{1}{2}\delta(-1) &\quad \text{otherwise}.
    \end{cases}$$
    Then we have
    \begin{align*}
        & \sum_{(\sx, \sa, r, \sx')\in\calX\times\calA\times\{-1, 1\}\times\calX}\mathbb{P}\ind{0}((\sx,\sa, r, \sx')) = \sum_{(\sx, \sa, \sx')\in\calX\times\calA\times\calX}\nu(\sx,\sa, \sx')\\
        &\quad = \sum_{\phi\in\Phi}\sum_{\phi'\in\Phi'}\sum_{\sz\in\phi}\sum_{\sz'\in\phi'}\mu(\sz, \sa)T\ind{1}(\sz'\mid \sz, \sa) = 1
    \end{align*}
    which indicates that $\mathbb{P}\ind{0}$ is a valid distribution. Additionally, \pref{lem:sec-lower-bound-latent-MDP} \ref{lem:sec-lower-bound-latent-MDP-c} gives that for any $\phi\in\Phi$, $\sz\in\calZ'$, we always have $\sum_{\sz\in\phi}\mu(\sz, \sa)T\ind{1}(\sz'\mid \sz, \sa) = \sum_{\sz\in\phi}\mu(\sz, \sa)T\ind{2}(\sz'\mid \sz, \sa)$. Therefore, the definition of $\mathbb{P}\ind{0}$ is symmetric between $M\ind{1}$ and $M\ind{2}$.

    If we prove
    $$\TV(\mathbb{P}_n\ind{1}, \mathbb{P}_n\ind{0})\le \frac{1}{4} \quad\text{and}\quad \TV(\mathbb{P}_n\ind{2}, \mathbb{P}_n\ind{0})\le \frac{1}{4},$$
    according to triangle inequality, we have $\TV(\mathbb{P}_n\ind{1}, \mathbb{P}_n\ind{2})\le \nicefrac{1}{2}$. Without loss of generality, in the following we  only prove
    $$\TV(\mathbb{P}_n\ind{1}, \mathbb{P}_n\ind{0})\le \frac{1}{4}.$$

    \paragraph{Part 1} In this part, we will first remove the dependence on reward functions. To achieve this, we define
    $$\tilde{\mathbb{P}}_n\ind{1}(\{(\sx_i,\sa_i, r_i, \sx_i')\}_{i=1}^n) = \frac{1}{|\Psi|}\sum_{\psi\in\Psi}\prod_{i=1}^n \rich{\mu}_\psi(\sx_i,\sa_i)\rich{R}\ind{0}(r_i \mid \sx_i,\sa_i)\rich{T}_{\psi}\ind{1}(\sx_i'\mid \sx_i,\sa_i).$$ 
    Next, we write
    $$\mathbb{P}_n\ind{1}(\{(\sx_i,\sa_i, r_i, \sx_i')\}_{i=1}^n) = \frac{1}{|\Psi|}\sum_{\psi\in\Psi}\prod_{i=1}^n \rich{\mu}_\psi(\sx_i,\sa_i)\rich{R}\ind{1}(r_i \mid \sx_i,\sa_i)\rich{T}_{\psi}\ind{1}(\sx_i'\mid \sx_i,\sa_i),$$
    where $\rich{R}\ind{1}$ is defined in \pref{eq:sec-lower-bound-def-r}. To facilitate the proof
    When $n\le \nicefrac{H\ophatC{M}{\mu}{\epsilon}{\Phi}}{2\epsilon}$, given the form of $\rich{r}\ind{0}$ and $\rich{r}\ind{1}$, we have
    \begin{align*}
        \TV(\mathbb{P}_n\ind{1}, \tilde{\mathbb{P}}_n\ind{1}) & = \frac{1}{2}\sum_{\{(\sx_i,\sa_i, r_i, \sx_i')\}_{i=1}^n}\left|\mathbb{P}_n\ind{1}(\{(\sx_i,\sa_i, r_i, \sx_i')\}_{i=1}^n - \tilde{\mathbb{P}}_n\ind{1}(\{(\sx_i,\sa_i, r_i, \sx_i')\}_{i=1}^n\right|\\
        &\le \frac{1}{2}\sum_{\{(\sx_i,\sa_i)\}_{i=1}^n}\frac{1}{|\Psi|}\sum_{\psi\in\Psi}\sum_{i=1}^n|\rich{r}\ind{1}(\sx_i,\sa_i) - \rich{r}\ind{0}(\sx_i,\sa_i)|\prod_{i=1}^n \rich{\mu}_\psi(\sx_i,\sa_i)\\
        &\le \frac{1}{2|\Psi|}\sum_{\psi\in\Psi}\sum_{i=1}^n\sum_{(\sx_i,\sa_i)}\rich{\mu}_\psi(\sx_i,\sa_i)|\rich{r}\ind{1}(\sx_i,\sa_i) - \rich{r}\ind{0}(\sx_i,\sa_i)|\\
        &\le \frac{1}{2|\Psi|}\sum_{\psi\in\Psi}\sum_{i=1}^n\sum_{\sx_i}\rich{\mu}_\psi(\sx_i, \ripieval(\sx_i))\frac{\epsilon\indic\{\zeta(\psi(\sx_i))\in\Phiopt)\}}{2H\sum_{\phi\in \Phiopt}d_h^\aggpieval(\phi; \agg{M})}\\
        & = \frac{n\epsilon}{4H\sum_{\phi\in \Phiopt}d_h^\aggpieval(\phi; \agg{M})}\sum_{\sz: \zeta(\sz)\in \Phiopt}\mu(\sz, \pieval(\sz))\le \frac{n\epsilon}{4H\ophatC{M}{\mu}{\epsilon}{\Phi}}\sum_{\phi\in \Phiopt} d_h^\aggpieval(\phi; \agg{M})\le \frac{1}{8}.
    \end{align*}

    Therefore, we obtain
    \begin{equation}\label{eq:sec-lower-bound-tv}\TV(\mathbb{P}_n\ind{1}, \mathbb{P}_n\ind{0})\le \TV(\mathbb{P}_n\ind{1}, \tilde{\mathbb{P}}_n\ind{1}) + \TV(\mathbb{P}_n\ind{0}, \tilde{\mathbb{P}}_n\ind{1})\le \frac{1}{8} + \TV(\mathbb{P}_n\ind{0}, \tilde{\mathbb{P}}_n\ind{1}).\end{equation}

    \paragraph{Part 2} In the next, we will try to bound $\TV(\mathbb{P}_n\ind{0}, \tilde{\mathbb{P}}_n\ind{1})$. First of all, we notice that
    $$\TV(\mathbb{P}_n\ind{0}, \tilde{\mathbb{P}}_n\ind{1})\le \frac{1}{2}\sqrt{D_{\chi^2}(\tilde{\mathbb{P}}_n\ind{1}\|\mathbb{P}_n\ind{0})}$$
    \ascomment{Where is this coming from?}  
    If using \(\mathbb{E}_{0}\) to denote \(\mathbb{E}_{\{(\sx_i,\sa_i, r_i, \sx_i')\}_{i=1}^n\sim \mathbb{P}_n\ind{0}}\), then we have
    \begin{align*}
        &\quad D_{\chi^2}(\tilde{\mathbb{P}}_n\ind{1}\|\mathbb{P}_n\ind{0}) \\ 
        & = \mathbb{E}_{0}\left[\left(\frac{\tilde{\mathbb{P}}_n\ind{1}(\{(\sx_i,\sa_i, r_i, \sx_i')\}_{i=1}^n)}{\mathbb{P}_n\ind{0}(\{(\sx_i,\sa_i, r_i, \sx_i')\}_{i=1}^n)}\right)^2\right] - 1\\
        & = \mathbb{E}_{0}\left[\left(\frac{\frac{1}{|\Psi|}\sum_{\psi\in\Psi}\prod_{i=1}^n \rich{\mu}_{\psi}(\sx_i,\sa_i)\rich{R}\ind{0}(r_i\mid\sx_i,\sa_i)\rich{T}_{\psi}\ind{1}(\sx_i'\mid \sx_i,\sa_i)}{\prod_{i=1}^n \nu(\sx_i, \sa_i,\sx_i')\rich{R}\ind{0}(r_i\mid\sx_i,\sa_i)}\right)^2\right] - 1\\
        & = \mathbb{E}_{0}\left[\left(\frac{\frac{1}{|\Psi|}\sum_{\psi\in\Psi}\prod_{i=1}^n \rich{\mu}_{\psi}(\sx_i,\sa_i)\rich{T}_{\psi}\ind{1}(\sx_i'\mid \sx_i,\sa_i)}{\prod_{i=1}^n \nu(\sx_i, \sa_i,\sx_i')}\right)^2\right] - 1\\
        & = \frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in \Psi}\mathbb{E}_{0}\left[\frac{\prod_{i=1}^n \rich{\mu}_{\psi_1}(\sx_i,\sa_i)\rich{\mu}_{\psi_2}(\sx_i,\sa_i)\rich{T}_{\psi_1}\ind{1}(\sx_i'\mid \sx_i,\sa_i)\rich{T}_{\psi_2}\ind{1}(\sx_i'\mid \sx_i,\sa_i)}{\prod_{i=1}^n\nu(\sx_i, \sa_i,\sx_i')^2}\right] - 1\\
        & = \frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in \Psi}\left(\mathbb{E}_{(\sx, \sa, \sx')\sim \nu}\left[\frac{\rich{\mu}_{\psi_1}(\sx,\sa)\rich{\mu}_{\psi_2}(\sx,\sa)\rich{T}_{\psi_1}\ind{1}(\sx'\mid \sx,\sa)\rich{T}_{\psi_2}\ind{1}(\sx'\mid \sx,\sa)}{\nu(\sx, \sa,\sx')^2}\right]\right)^n - 1
    \end{align*}

    Next, using Jensen's inequality, we can separate the above equation into sum over $\phi$ and $\phi'$:
    \begin{align*}
        & \le \mathbb{E}_{h\in[H-1]}\mathbb{E}_{\phi\in \Phi_h, \phi'\in\Phi_{h+1}\cup\{\su_{h+1}, \sv_{h+1}\}, \sa\in\calA} \\
        & \quad \frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in\Psi}\left(\mathbb{E}_{(\sx, \sx')\sim \nu(\cdot\mid \phi, \phi', \sa)}\left[\frac{\rich{\mu}_{\psi_1}(\sx\mid\phi, \sa)\rich{\mu}_{\psi_2}(\sx\mid \phi, \sa)\rich{T}_{\psi_1}\ind{1}(\sx'\mid \sx,\sa, \phi')\rich{T}_{\psi_2}\ind{1}(\sx'\mid \sx,\sa, \phi')}{\nu(\sx,\sx'\mid \phi, \phi', \sa)^2}\right]\right)^n - 1
    \end{align*}
    In the following, we will upper bound the term in the expectation one-by-one.


    \paragraph{Part 3} In this part, we fix $h\in [H-1], \phi, \phi'$ and $\sa$. We define
    $$\theta_{\sz_1, \sz_2}(\psi_1, \psi_2)\triangleq \frac{|\calX_{\psi_1}(\sz_1)\cap \calX_{\psi_2}(\sz_2)|}{|\calX(\phi)|},\quad \forall \sz_1, \sz_2\in \phi.$$
    We further define sets 
    \begin{equation}\label{eq:sec-lower-bound-defGamma}\Gamma_{\phi, \sz_1, \sz_2}(\xi)\triangleq \left\{(\psi_1, \psi_2): \theta_{\sz_1, \sz_2}\le \frac{1 + \xi}{|\phi|^2}\right\},\quad \Gamma_\phi(\xi) = \bigcap_{\sz_1, \sz_2\in \phi}\Gamma_{\phi, \sz_1, \sz_2}(\xi),\quad\text{and}\quad \Gamma(\xi) = \bigcap_{\phi\in\Phi}\Gamma_\phi(\xi).\end{equation}
    For those $\sx\in \calX_{\psi_1}(\sz_1)\cap \calX_{\psi_2}(\sz_2)$, we have
    \begin{align*}
        \rich{\mu}_{\psi_1}(\sx\mid\phi, \sa) = \frac{\mu(\sz_1\mid\phi, \sa)}{|\calX_{\psi_1}(\sz_1)|} = \frac{\mu(\sz_1\mid, \phi, \sa)|\phi|}{|\calX(\phi)|}\quad\text{and}\quad\rich{\mu}_{\psi_2}(\sx\mid\phi, \sa) = \frac{\mu(\sz_2\mid\phi, \sa)|\phi|}{|\calX(\phi)|}.
    \end{align*}
    For $\sx'\in\calX_{\psi_1}(\sz_1')\cap \calX_{\psi_2}(\sz_2')$, we also have
    $$\rich{T}_{\psi_1}\ind{1}(\sx'\mid \sx,\sa, \phi') = \frac{T\ind{1}(\sz_1'\mid\sz_1, \sa, \phi')|\phi'|}{|\calX(\phi')|}\quad\text{and}\quad\rich{T}_{\psi_2}\ind{1}(\sx'\mid \sx,\sa, \phi') = \frac{T\ind{1}(\sz_2'\mid\sz_2, \sa, \phi')|\phi'|}{|\calX(\phi')|}.$$
    Additionally, \pref{eq:sec-lower-bound-def-nu} gives that
    $$\nu(\sx, \sa, \sx'\mid \phi, \phi', \sa) = \frac{1}{|\calX(\phi)||\calX(\phi')|}.$$
    
    


    We first analyze the case where $\phi'\not\in\{\su_h, \sv_h\}_{h=1}^H$. For any $(\psi_1, \psi_2)\in \Gamma(\xi)$, we have
    \begin{align*} 
        &\quad \mathbb{E}_{(\sx, \sx')\sim \nu(\cdot\mid \phi, \phi', \sa)}\left[\frac{\rich{\mu}_{\psi_1}(\sx\mid\phi, \sa)\rich{\mu}_{\psi_2}(\sx\mid \phi, \sa)\rich{T}_{\psi_1}\ind{1}(\sx'\mid \sx,\sa, \phi')\rich{T}_{\psi_2}\ind{1}(\sx'\mid \sx,\sa, \phi')}{\nu(\sx,\sx'\mid \phi, \phi', \sa)^2}\right]\\
        & = \sum_{\sx\in\phi, \sx'\in\phi'}\frac{\rich{\mu}_{\psi_1}(\sx\mid\phi, \sa)\rich{\mu}_{\psi_2}(\sx\mid \phi, \sa)\rich{T}_{\psi_1}\ind{1}(\sx'\mid \sx,\sa, \phi')\rich{T}_{\psi_2}\ind{1}(\sx'\mid \sx,\sa, \phi')}{\nu(\sx,\sx'\mid \phi, \phi', \sa)}\\
        & = \sum_{\sz_1, \sz_2\in\phi}\sum_{\sz_1', \sz_2'\in\phi'}\sum_{\sx\in \calX_{\psi_1}(\sz_1)\cap \calX_{\psi_2}(\sz_2)}\sum_{\sx'\in\calX_{\psi_1}(\sz_1')\cap \calX_{\psi_2}(\sz_2')}\frac{\rich{\mu}_{\psi_1}(\sx\mid\phi, \sa)\rich{\mu}_{\psi_2}(\sx\mid \phi, \sa)\rich{T}_{\psi_1}\ind{1}(\sx'\mid \sx,\sa, \phi')\rich{T}_{\psi_2}\ind{1}(\sx'\mid \sx,\sa, \phi')}{\nu(\sx,\sx'\mid \phi, \phi', \sa)}\\
        & = \sum_{\sz_1, \sz_2\in\phi}\sum_{\sz_1', \sz_2'\in\phi'}\theta_{\sz_1, \sz_2}(\psi_1, \psi_2)|\calX(\phi)|\cdot \theta_{\sz_1', \sz_2'}(\psi_1, \psi_2)|\calX(\phi')|\\
        &\qquad \cdot \frac{\mu(\sz_1\mid\phi, \sa)\mu(\sz_2\mid\phi, \sa)T\ind{1}(\sz_1'\mid\sz_1, \sa, \phi')T\ind{1}(\sz_2'\mid\sz_2, \sa, \phi')\cdot |\phi|^2|\phi'|^2}{|\calX(\phi)||\calX(\phi')|}\\
        &\le \sum_{\sz_1, \sz_2\in\phi}\sum_{\sz_1', \sz_2'\in\phi'} (1 + \xi)^2\cdot\mu(\sz_1\mid\phi, \sa)\mu(\sz_2\mid\phi, \sa)T\ind{1}(\sz_1'\mid\sz_1, \sa, \phi')T\ind{1}(\sz_2'\mid\sz_2, \sa, \phi') = (1 + \xi)^2,
    \end{align*} 
    where in the inequality we use the fact that $(\psi_1, \psi_2)\in\Gamma(\xi)$.

    Additionally, for any $(\psi_1, \psi_2)\in \Psi^2$, noticing that $\theta_{\sz_1, \sz_2}\le 1$ always holds for all $\sz_1, \sz_2$, we have
    \begin{align*}
        &\quad \mathbb{E}_{(\sx, \sx')\sim \nu(\cdot\mid \phi, \phi', \sa)}\left[\frac{\rich{\mu}_{\psi_1}(\sx\mid\phi, \sa)\rich{\mu}_{\psi_2}(\sx\mid \phi, \sa)\rich{T}_{\psi_1}\ind{1}(\sx'\mid \sx,\sa, \phi')\rich{T}_{\psi_2}\ind{1}(\sx'\mid \sx,\sa, \phi')}{\nu(\sx,\sx'\mid \phi, \phi', \sa)^2}\right]\\
        &\le \sum_{\sz_1, \sz_2\in\phi}\sum_{\sz_1', \sz_2'\in\phi'}\theta_{\sz_1, \sz_2}(\psi_1, \psi_2)\theta_{\sz_1', \sz_2'}(\psi_1, \psi_2)\mu(\sz_1\mid\phi, \sa)\mu(\sz_2\mid\phi, \sa)T\ind{1}(\sz_1'\mid\sz_1, \sa, \phi')T\ind{1}(\sz_2'\mid\sz_2, \sa, \phi')\cdot |\phi|^2|\phi'|^2\\
        & = |\phi|^2|\phi'|^2.
    \end{align*}
    Therefore, we obtain that
    \begin{align*}
        &\quad \frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in\Psi}\left(\mathbb{E}_{(\sx, \sx')\sim \nu(\cdot\mid \phi, \phi', \sa)}\left[\frac{\rich{\mu}_{\psi_1}(\sx\mid\phi, \sa)\rich{\mu}_{\psi_2}(\sx\mid \phi, \sa)\rich{T}_{\psi_1}\ind{1}(\sx'\mid \sx,\sa, \phi')\rich{T}_{\psi_2}\ind{1}(\sx'\mid \sx,\sa, \phi')}{\nu(\sx,\sx'\mid \phi, \phi', \sa)^2}\right]\right)^n - 1\\
        & \le \frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in \Psi} \left[(1 + \xi)^n + \indic\{(\psi_1, \psi_2)\not\in \Gamma(\xi)\}|\phi|^{2n}|\phi'|^{2n}\right] - 1.
    \end{align*}
    When $\xi \le \nicefrac{1}{n}$, we have $(1 + \xi)^n \le 1 + 2\xi n$, which indicates that the above formula is 
    $$\le 2\xi n + |\phi|^{2n}|\phi'|^{2n}\frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in \Psi}\indic\{(\psi_1, \psi_2)\not\in \Gamma(\xi)\}.$$
    Next, according to Lemma \ref{lem:g_phi}, we have
    $$\frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in \Psi} \indic\{\psi_1, \psi_2)\not\in \Gamma_{\phi, \sz_1, \sz_2}(\xi)\} \le \exp(\nicefrac{-2\xi^2 |\calX(\phi)|}{|\phi|}).$$
    Hence,
    $$\frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in \Psi}\indic\{(\psi_1, \psi_2)\not\in \Gamma(\xi)\}\le |\Phi|\sup_{\phi\in\Phi}|\phi|^2\exp(\nicefrac{-2\xi^2 |\calX(\phi)|}{|\phi|}).$$
    When $|\calX(\phi)|\ge \nicefrac{32|\phi|^4H^3\ophatC{M}{\mu}{\epsilon}{\Phi}^3}{\epsilon^3}$ and $n\le \nicefrac{H\ophatC{M}{\mu}{\epsilon}{\Phi}}{8\epsilon}$, we have
    $$|\calX(\phi)|\ge 16384|\phi|^4n^3\ge 8192|\phi|^4n^2 + 4096(n+1)|\phi|^3n^2\log|\phi|.$$
    Hence if we choose $\xi = \nicefrac{1}{64|\phi|n}$, we obtain
    $$2|\phi|\xi n + |\phi|^{2n}\frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in \Psi}\indic\{(\psi_1, \psi_2)\not\in \Gamma_\phi(\xi)\}\le 2|\phi|\xi n + |\phi|^2\exp(\nicefrac{-2\xi^2 |\calX(\phi)|}{|\phi|})\le \frac{1}{16}.$$
    This indicate that
    $$\frac{1}{|\Psi|^2}\sum_{\psi_1, \psi_2\in \Psi}\left(\mathbb{E}_{\sx\sim \rich{\mu}\ind{0}(\cdot\mid \phi, \sa), \sx'\in \rich{T}\ind{0}(\cdot\mid \sx, \sa)}\left[\frac{\rich{\mu}_{\psi_1}(\sx\mid \phi, \sa)\rich{\mu}_{\psi_2}(\sx\mid \phi, \sa)\rich{T}_{\psi_1}\ind{1}(\sx'\mid \sx,\sa)\rich{T}_{\psi_2}\ind{1}(\sx'\mid \sx,\sa)}{\rich{\mu}\ind{0}(\sx\mid \phi, \sa)^2\rich{T}\ind{0}(\sx'\mid \sx,\sa)^2}\right]\right)^n - 1\le \frac{1}{16},$$
    and hence 
    $$D_{\chi^2}(\tilde{\mathbb{P}}_n\ind{1}\|\mathbb{P}_n\ind{0})\le \frac{1}{16}.$$
    Bringing this inequality back into \pref{eq:sec-lower-bound-tv}, we have
    $$\TV(\mathbb{P}_n\ind{1}~\|~\mathbb{P}_n\ind{0})\le \frac{1}{4}.$$
    This completes the proof of this lemma.
\end{proof}

==> files/results_overview.tex <==
\section{Overview of Results} 
In this paper, we provide both upper and lower bounds. We start with the overview of our main lower bound first. 

\paragraph{Lower Bounds}
\begin{theorem}[Informal] For all feasible\footnote{From feasible, we mean that there exist an MDP and aggregation scheme \(\Phi\) that realized it \ascomment{Complete this!}}  $C$ and $\bar{C}$, there exists a family of MDPs \(\cM\) such that every MDP in this family 
has concentrability $C$ and aggregated concentrability \(\bar{C}\) such that any offline RL algorithm needs \[\Omega(\bar{C}/\epsilon)\] samples in some MDP in this family. 
%, with standard concentrability \(C\) and aggregated concentrability \(\bar{C}\), with \(C \neq \bar{C}\) such that any offline RL algorithm needs \(\Omega(\bar{C}/\epsilon)\) samples in some MDP in this family. 
\end{theorem}

Notice that the lower bound depends on \(\bar{C}\) instead of C, as one might expect. In fact, as we show next the gap between  \(\bar{C}\) and \(C\) could be huge. 

\begin{theorem} There exists an offline distribution \(\mu\) and an MDP $M$ such that with \(C = O(H)\) and \(\bar{C} = O(2^H)\). Furthermore, \(\mu\) is an admissible distribution for $M$. 
\ascomment{Shows that there is a gap between $C$ and $\bar{C}$}
\end{theorem}

\begin{lemma}\ascomment{Make it a corrollary}
    [Admissible Data Separation] There exists a family of MDPs  with concentrability \(C = O(H)\)  such that any offline algorithm needs 
\[\Omega(2^H/\epsilon)\] samples. 
\end{lemma}

\ascomment{Discussion on admissible vs trajectory again; prior conjecture and that we show that it is false in the following }

\begin{theorem}[Lower bound against trajectory offline data] 

    There exists a family of MDPs and trajectory data \(\mu\)  with concentrability \(C = O(H)\)  such that any offline algorithm needs 
\[\Omega(2^H/\epsilon)\] samples. 
\end{theorem}

\ascomment{Paragraph about reduction of trajectory to admissible with appropriate pointers!} 

The key idea was that \(\bar{C}\) is what dictates the lower bound. In fact, first theorem above was shown via a general purpose reduction that lifts any MDPs (give a point to it) .... 

Is bounded \(\bar{C}\)  also sufficient ?

\paragraph{Upper Bound.} 
\begin{theorem}[Informal; formal version given in ] Upper Bound 
\end{theorem}

The above upper bound is obtained using a slight variant of seminal work of Tengyang : BVFT algorithm. 

\paragraph{Role of Function Approximation.}  

Inline paragraph/theorems. 

==> files/sketch.tex <==
\ascomment{Should be removed from the final version of the paper!!} 

\iffalse  %%%% Sasha's sketch 
\section{Sketch} 

\begin{enumerate}
    \item Introduction
    \item Preliminaries 
    \item Overview of Results 
    \begin{enumerate}
        \item Theorem: Instantiation of Trajectory Lower Bound. 
        \item Paragraph discussion of how to obtain this. 
        \begin{enumerate}
            \item Reduction from Admissible to trajectory. 
            \item Crisp Theorem: Lower Bound for Admissible.  
        \end{enumerate}
        \item In-fact, what determines the rate is not concentrability but aggregated concentrability. 
        \item Informal Theorem. 
        \item Upper Bound that parallels this theorem. 
    \end{enumerate}
    \item Admissible to Trajectory reduction. 
    \item General lower bound for admissible data. 
    \item Given lower bound construction and why aggregated concentrability is large / Add a picture. 
    \item Upper Bound  
\end{enumerate}
\fi 


\clearpage 

\section{Introduction}
\section{Related Works}
\section{Preliminaries}
\section{Overview of Results}
\section{Lower Bounds}\label{sec: lower bound}

\subsection{A General Lower Bound}  
\begin{theorem} Full-fledged general reduction for general data. 
\end{theorem}


\subsubsection{Why aggregated concentrability? From Tabular MDPs to function approximation.}   
\ascomment{Chenyu's discussion modified to explain why \(\bar{C}\) matters?}

\subsubsection{Proof Sketch} 
\ascomment{Max 2.5 pages with figures.} 

\subsection{Lower Bound for Admissible Data}
Show example here! 

\subsection{Lower Bound for Trajectory Data}  
Actual theorem and reduction 

\section{Upper Bound} 

\section{From policy evaluation to learning} 

\section{Role of function class} 

\section{Conclusion}


\clearpage 





==> notes.tex <==
\begin{enumerate} 
\item 08/13
\begin{enumerate}
\item Alternate clipping strategies, e.g. by thresholding. 
\item Hybrid RL setting. 
\item General reductions. 
\end{enumerate} 

\item 06/12 
\begin{enumerate}
\item Discussion on \(\min-\max\) vs \(\max-\max\) for bandits. 
\item \textbf{PRO-RL:} 
\begin{enumerate}
\item Make modeling assumptions about \(d^\pi\). Two versions: 
\begin{enumerate}
\item \(d^\pi \in \cD\) for all \(\pi \in \Pi\). 
\item The mapping \(\crl{\pi \mapsto d^\pi \in \cG}\) where \(\cG\) is a mapping class. 
\end{enumerate}
\end{enumerate}

\item \textbf{LOWER BOUND:}  Can we show that just weight function realizability is not sufficient for efficient algorithm (I guess the lower bound here should be a statistical lower bound). The exact assumptions that we consider are: 
\begin{enumerate} 
\item \(d^{\pistar}/d^\pi \in \cW\) for all \(\pi \in \Pi\). 
\item Coverability 
\item \(V^\pi \in \cV\) for all \(\pi \in \Pi\) 
\end{enumerate}
Can start with a bandit problem here for the lower bound. 

\item \textbf{FORCE:} 
\begin{enumerate}
\item Can we see if there is a benefit of their clipping strategy for our analysis? 
\item Trivial extension: Getting FORCE to work under coverability.  
\item Is there a relation between forward completeness and backward completeness? Is one simpler than the other? 
\item Two version of completness: (a) completeness for any function \(d\), (b) completeness for valid occupancy measures ($P d \in \cD$). Generally, layer-by-layer approaches e.g. LSVI require (a), and global algorithms like GOLF require (b). The current version of FORCE requires (a), but is there a way to make it ``GOLF like" so that it can work with (b) style assumption.  \\

(b) is a weaker statistical assumption as compared to (a), and layer-by-layer approach is a proxy for computational efficiency. 
\item Other questions that we discussed: 
\begin{enumerate}
\item Can we show a lower bound showing that linear-Bellman complete is computationally intractable?
\item There is a reward free version of GOLF in \cite{xie2022role}. What should be the reward class that we should feed into it so that the returned policies by this reward-free algorithm is exploratory, i.e. has good coverage. 
\item Can we get a reward free version of our current \(Q\)-function based algorithm? Can this be actually made efficient (generally we can get efficient algorithms if we do not have the optimism term in olive, e.g. done by Rewardfree OLIVE)?  
\item 
\end{enumerate}

\end{enumerate}

\end{enumerate}

\item 05/30 
\begin{enumerate}
\item \textbf{Online RL: First Algorithm:} 
\begin{enumerate}
\item \(Q^\star \in \cF\) 
\item \(\frac{d^{\pi}}{d^{\bar \pi}} \in \cW\)  for all \(\pi \in \Pi\). 
\end{enumerate}
This algorithm is computationally efficient as it needs a joint optimization step over \(\cF\) similar in spirit to Golf. 
\item \textbf{Offline RL: ProRL based algorithm}  
\begin{enumerate}
\item $v^\pi \in \cV$ for all \(\pi\) 
\item Single policy concentrability \(C_\pistar\) and realizability: \(\frac{d^{\pi^\star}}{\nu} \in \cV\)  
\end{enumerate}
Computationally efficient algorithm. Under the assumption that we have access to an offline data distribution \(\nu\) from which we can sample \(\sa\), we can convert the above into an efficient online algorithm. 
\item Another idea to explore is whether we can replace coverage by known \(\nu \) + single policy concentrability in online RL. 
\item 
\end{enumerate} 

\item 04/15  
\begin{enumerate}
\item Can Maurey sparsification help us in getting a \(\sqrt{T}\) regret bound? 
\item Verify why is the current algorithm no simpler than Olive, but is simpler than GOLF? 
\end{enumerate}

\end{enumerate}

\begin{enumerate}
\item Can we add Bellman error times weight inside the indictor. Like \(\indicator{w(s, a) }\)
\item Weight function class in latent space + Value function class => Weight function class + Value function class in Rich Observation RL. 
\end{enumerate}



==> todonotes.tex <==
% Todonotes
\usepackage[colorinlistoftodos,prependcaption,textsize=scriptsize]{todonotes} %\usepackage{xargs} % to use more than one optional parameter in a new commands
\providecommand{\tdotoggle}{1}
 \ifnum\tdotoggle=1
 \setlength{\marginparwidth}{1.5cm}
 \paperwidth=\dimexpr \paperwidth + 3.2cm\relax
 \oddsidemargin=\dimexpr\oddsidemargin + 1.6cm\relax
 \evensidemargin=\dimexpr\evensidemargin + 1.6cm\relax
 \marginparwidth=\dimexpr \marginparwidth + 1.6cm\relax
 \fi
\newcommand{\mytodo}[1]{\ifnum\tdotoggle=1{#1}\fi}
\newcommand{\mynote}[1]{\mytodo{\textcolor{Gred}{#1}}}
\newcommand{\mycomment}[1]{{\color{Gred}{$\langle$#1$\rangle$}} \addcontentsline{tdo}{todo}{#1}}
\newcommand{\todoinline}[1]{\mytodo{\todo[inline,linecolor=Gred,backgroundcolor=Gred!25,bordercolor=Gred]{#1}}}
\newcommand{\improve}[1]{\mytodo{\todo[linecolor=myBlue,backgroundcolor=myBlue!25,bordercolor=myBlue]{#1}}}
\newcommand{\unsure}[1]{\mytodo{\todo[linecolor=myGold,backgroundcolor=myGold!25,bordercolor=myGold]{#1}}}
\newcommand{\info}[1]{\mytodo{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen]{#1}}}
\newcommand{\change}[1]{\mytodo{\todo[linecolor=Gred,backgroundcolor=Gred!25,bordercolor=Gred]{#1}}}
\newcommand{\tableoftodos}{\ifnum\tdotoggle=1 \listoftodos[Comments/To Do's] \fi}

% Add bubble here
\newcommand{\cw}[1]{\mytodo{\todo[linecolor=Ggreen,backgroundcolor=Ggreen!25,bordercolor=Ggreen]{Gene: #1}}}

\newcommand{\ayush}[1]{\mytodo{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{Ayush: #1}}}

\newcommand{\sasha}[1]{\mytodo{\todo[linecolor=blue,backgroundcolor=purple!25,bordercolor=purple]{Sasha: #1}}}


\newcommand{\zeyu}[1]{\mytodo{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red]{Zeyu: #1}}}


% Custom Colors
\definecolor{Gred}{RGB}{219, 50, 54}
\definecolor{Ggreen}{RGB}{60, 186, 84}
\definecolor{Gblue}{RGB}{72, 133, 237}
\definecolor{Gyellow}{RGB}{247, 178, 16}
\definecolor{ToCgreen}{RGB}{0, 128, 0}
\definecolor{myGold}{RGB}{231,141,20}
\definecolor{myBlue}{rgb}{0.19,0.41,.65}
\definecolor{myPurple}{RGB}{175,0,124}
